Idoneal genera and K3 surfaces covering an Enriques surface

Idoneal genera are a generalization of Euler's idoneal numbers. We enumerate all idoneal genera by means of the Smith--Minkowski--Siegel mass formula. As an application, we classify transcendental lattices of K3 surfaces covering an Enriques surface.

==> tabs/half_co-id.tex <==
\begin{center}
\renewcommand{\arraystretch}{1.2}
%\small
%\scriptsize
\footnotesize

\begin{longtable}{llll}
  \caption{Halves of co-idoneal lattices (see \autoref{thm:co-idoneal}), listed by increasing rank \(\lambda = \rank T'\) and determinant.}
  \label{tab:half_co-id} \\
  
    \toprule
        $\lambda$ & No. & $\det T'$ & $T'$ \\
    \midrule
  \endfirsthead

    \multicolumn{4}{c}%
    {\tablename\ \thetable{}, continued from previous page.} \\
    \midrule
        $\lambda$ & No. & $\det T'$ & $T'$ \\
    \midrule
  \endhead

    \multicolumn{4}{c}{Continued on next page.} \\ \midrule
  \endfoot

    \bottomrule
  \endlastfoot

 \(2\) & \(1\) & \(1\) & \(2 [1]\) \\
 \(2\) & \(2\) & \(2\) & \([1] \oplus [2]\) \\
 \(2\) & \(3\) & \(4\) & \([1] \oplus [4]\) \\
\midrule
 \(3\) & \(1\) & \(-1\) & \([1] \oplus \bU\) \\
 \(3\) & \(2\) & \(-2\) & \([1] \oplus [2] \oplus [-1]\) \\
 \(3\) & \(3\) & \(-3\) & \(2 [1] \oplus [-3]\) \\
 \(3\) & \(4\) & \(-4\) & \([1] \oplus [2] \oplus [-2]\) \\
 \(3\) & \(5\) & \(-4\) & \([1] \oplus \bU(2)\) \\
 \(3\) & \(6\) & \(-5\) & \([1] \oplus [2, 1, -2]\) \\
 \(3\) & \(7\) & \(-8\) & \([2] \oplus [0, 2, -1]\) \\
 \(3\) & \(8\) & \(-9\) & \([-1] \oplus 2 [3]\) \\
\midrule
 \(4\) & \(1\) & \(1\) & \(2 [1] \oplus 2 [-1]\) \\
 \(4\) & \(2\) & \(2\) & \([1] \oplus [-2] \oplus \bU\) \\
 \(4\) & \(3\) & \(3\) & \([-1] \oplus [3] \oplus \bU\) \\
 \(4\) & \(4\) & \(4\) & \([1] \oplus [-1, 1, 1, -1, 1, 1](-1)\) \\
 \(4\) & \(5\) & \(4\) & \([1] \oplus [-1] \oplus \bU(2)\) \\
 \(4\) & \(6\) & \(4\) & \([1] \oplus [-1] \oplus [0, 2, -1]\) \\
 \(4\) & \(7\) & \(4\) & \([1] \oplus [-1] \oplus [0, 2, 1]\) \\
 \(4\) & \(8\) & \(5\) & \([-1] \oplus [1] \oplus [2, 1, -2]\) \\
 \(4\) & \(9\) & \(6\) & \([1] \oplus [1, 2, -1, 0, 1, 1](-1)\) \\
 \(4\) & \(10\) & \(8\) & \([1] \oplus [2] \oplus 2 [-2]\) \\
 \(4\) & \(11\) & \(8\) & \([1] \oplus [-2, 1, 2, 0, 1, 2](-1)\) \\
 \(4\) & \(12\) & \(9\) & \([3] \oplus [-3] \oplus \bU\) \\
 \(4\) & \(13\) & \(9\) & \([0, 3, 2, 0, 2, 0, 0, -5, 1, 1]\) \\
 \(4\) & \(14\) & \(12\) & \([3] \oplus [0, 2, -2, 0, 1, 1](-1)\) \\
 \(4\) & \(15\) & \(16\) & \([-4] \oplus [0, 2, 1, 0, 1, 1]\) \\
 \(4\) & \(16\) & \(16\) & \([4] \oplus [0, 2, 1, 0, 1, 1](-1)\) \\
 \(4\) & \(17\) & \(16\) & \([1] \oplus [-1] \oplus \bU(4)\) \\
\midrule
 \(5\) & \(1\) & \(-1\) & \([-1] \oplus 2 \bU\) \\
 \(5\) & \(2\) & \(-2\) & \([1] \oplus [-1] \oplus [-2] \oplus \bU\) \\
 \(5\) & \(3\) & \(-3\) & \(2 [-1] \oplus [3] \oplus \bU\) \\
 \(5\) & \(4\) & \(-3\) & \([1] \oplus [-1] \oplus [-3] \oplus \bU\) \\
 \(5\) & \(5\) & \(-4\) & \([1] \oplus 2[-1] \oplus [2] \oplus [-2]\) \\
 \(5\) & \(6\) & \(-4\) & \([-1] \oplus \bU \oplus \bU(2)\) \\
 \(5\) & \(7\) & \(-4\) & \([1] \oplus [-1] \oplus [-4] \oplus \bU\) \\
 \(5\) & \(8\) & \(-4\) & \([-1] \oplus \bU \oplus [-1, 1, 3]\) \\
 \(5\) & \(9\) & \(-5\) & \(2 [-1] \oplus [5] \oplus \bU\) \\
 \(5\) & \(10\) & \(-6\) & \([1] \oplus [-1] \oplus [-6] \oplus \bU\) \\
 \(5\) & \(11\) & \(-7\) & \([-1] \oplus \bU \oplus [2, 1, -3]\) \\
 \(5\) & \(12\) & \(-7\) & \(2 [-1] \oplus [7] \oplus \bU\) \\
 \(5\) & \(13\) & \(-8\) & \([1] \oplus [-1] \oplus [-2] \oplus \bU(2)\) \\
 \(5\) & \(14\) & \(-8\) & \([-1] \oplus [-2] \oplus [4] \oplus \bU\) \\
 \(5\) & \(15\) & \(-8\) & \(2 [-1] \oplus [8] \oplus \bU\) \\
 \(5\) & \(16\) & \(-8\) & \([-1] \oplus [1] \oplus [0, 2, -2, 0, 1, 2](-1)\) \\
 \(5\) & \(17\) & \(-8\) & \([1] \oplus [-1] \oplus [-8] \oplus \bU\) \\
 \(5\) & \(18\) & \(-9\) & \(\bU \oplus [0, 3, -2, 0, 1, 1](-1)\) \\
 \(5\) & \(19\) & \(-9\) & \([0, 3, 2, 0, 1, 0, 0, 1, 0, 1, 0, 1, 1, 0, 0](-1)\) \\
 \(5\) & \(20\) & \(-10\) & \([1] \oplus [-1] \oplus [-10] \oplus \bU\) \\
 \(5\) & \(21\) & \(-12\) & \([1] \oplus [-1] \oplus [-3] \oplus \bU(2)\) \\
 \(5\) & \(22\) & \(-12\) & \(2 [-1] \oplus [3] \oplus \bU(2)\) \\
 \(5\) & \(23\) & \(-12\) & \(2[-1] \oplus [1] \oplus [2, 1, -1](2)\) \\
 \(5\) & \(24\) & \(-12\) & \([-1] \oplus [-3] \oplus [4] \oplus \bU\) \\
 \(5\) & \(25\) & \(-13\) & \(2 [-1] \oplus [13] \oplus \bU\) \\
 \(5\) & \(26\) & \(-15\) & \([3] \oplus \bU \oplus [2, 1, 3](-1)\) \\
 \(5\) & \(27\) & \(-16\) & \([-1] \oplus 2 \bU(2)\) \\
 \(5\) & \(28\) & \(-16\) & \([1] \oplus [-1] \oplus [-4] \oplus \bU(2)\) \\
 \(5\) & \(29\) & \(-16\) & \([1] \oplus 2 [-4] \oplus \bU\) \\
 \(5\) & \(30\) & \(-16\) & \([0, 2, -2, 0, 1, 1, 0, 1, 0, -2, 0, 1, 0, 0, 2](-1)\) \\
 \(5\) & \(31\) & \(-16\) & \([-4] \oplus \bU \oplus [-1, 1, 3]\) \\
 \(5\) & \(32\) & \(-16\) & \([1] \oplus [-1] \oplus [-16] \oplus \bU\) \\
 \(5\) & \(33\) & \(-18\) & \([-1] \oplus [-2] \oplus [9] \oplus \bU\) \\
 \(5\) & \(34\) & \(-20\) & \(2 [-1] \oplus [5] \oplus \bU(2)\) \\
 \(5\) & \(35\) & \(-21\) & \([-1] \oplus [-3] \oplus [7] \oplus \bU\) \\
 \(5\) & \(36\) & \(-24\) & \([1] \oplus [-1] \oplus [-24] \oplus \bU\) \\
 \(5\) & \(37\) & \(-27\) & \([1] \oplus [-1] \oplus [3] \oplus 2[-3]\) \\
 \(5\) & \(38\) & \(-32\) & \([1] \oplus [-1] \oplus [-2] \oplus \bU(4)\) \\
 \(5\) & \(39\) & \(-32\) & \([1] \oplus [-1] \oplus [-8] \oplus \bU(2)\) \\
 \(5\) & \(40\) & \(-48\) & \(\bU(2) \oplus [0, 2, -1, 0, 1, 3](-1)\) \\
 \(5\) & \(41\) & \(-64\) & \([1] \oplus 2 [-4] \oplus \bU(2)\) \\
\midrule
 \(6\) & \(1\) & \(1\) & \(2 [-1] \oplus 2 \bU\) \\
 \(6\) & \(2\) & \(2\) & \(2 [-1] \oplus [1] \oplus [-2] \oplus \bU\) \\
 \(6\) & \(3\) & \(3\) & \([-1] \oplus [-3] \oplus 2 \bU\) \\
 \(6\) & \(4\) & \(3\) & \([1] \oplus [-1] \oplus \bU \oplus \bA_{2}\) \\
 \(6\) & \(5\) & \(4\) & \([1] \oplus [-1] \oplus 2 [-2] \oplus \bU\) \\
 \(6\) & \(6\) & \(4\) & \(2 [-1] \oplus \bU \oplus \bU(2)\) \\
 \(6\) & \(7\) & \(4\) & \(2 [-1] \oplus \bU \oplus [0, 2, -1]\) \\
 \(6\) & \(8\) & \(4\) & \([-1] \oplus [-4] \oplus 2 \bU\) \\
 \(6\) & \(9\) & \(5\) & \(3 [-1] \oplus [5] \oplus \bU\) \\
 \(6\) & \(10\) & \(5\) & \(2 \bU \oplus [2, 1, 3](-1)\) \\
 \(6\) & \(11\) & \(6\) & \(2 [-1] \oplus [-2] \oplus [3] \oplus \bU\) \\
 \(6\) & \(12\) & \(6\) & \([1] \oplus [-1] \oplus [-2] \oplus [-3] \oplus \bU\) \\
 \(6\) & \(13\) & \(7\) & \([1] \oplus 2[-1] \oplus [-7] \oplus \bU\) \\
 \(6\) & \(14\) & \(8\) & \([-1] \oplus [-2] \oplus \bU(2) \oplus \bU\) \\
 \(6\) & \(15\) & \(8\) & \(2 [-1] \oplus [-2] \oplus [4] \oplus \bU\) \\
 \(6\) & \(16\) & \(8\) & \(3 [-1] \oplus [8] \oplus \bU\) \\
 \(6\) & \(17\) & \(8\) & \([-1] \oplus [1] \oplus \bU \oplus [3, 1, 3](-1)\) \\
 \(6\) & \(18\) & \(8\) & \([-1] \oplus [-8] \oplus 2 \bU\) \\
 \(6\) & \(19\) & \(9\) & \([1] \oplus [-1] \oplus 2 [-3] \oplus \bU\) \\
 \(6\) & \(20\) & \(9\) & \(2 [-1] \oplus \bU \oplus [-2, 1, 4]\) \\
 \(6\) & \(21\) & \(9\) & \(3 [-1] \oplus [9] \oplus \bU\) \\
 \(6\) & \(22\) & \(10\) & \(2 [-1] \oplus [-2] \oplus [5] \oplus \bU\) \\
 \(6\) & \(23\) & \(11\) & \([-1] \oplus [1] \oplus \bU \oplus [3, 1, 4](-1)\) \\
 \(6\) & \(24\) & \(11\) & \([1] \oplus [-1] \oplus [-2, 1, 2, 0, 1, 2, 0, 1, 1, 2](-1)\) \\
 \(6\) & \(25\) & \(12\) & \([1] \oplus [-1] \oplus \bU(2) \oplus \bA_{2}\) \\
 \(6\) & \(26\) & \(12\) & \([1] \oplus [-1] \oplus [-2] \oplus [-6] \oplus \bU\) \\
 \(6\) & \(27\) & \(12\) & \([-1] \oplus [-3] \oplus \bU \oplus \bU(2)\) \\
 \(6\) & \(28\) & \(12\) & \([1] \oplus [-1] \oplus [-3] \oplus [-4] \oplus \bU\) \\
 \(6\) & \(29\) & \(12\) & \([1] \oplus [-4] \oplus \bU \oplus \bA_{2}\) \\
 \(6\) & \(30\) & \(12\) & \([1] \oplus 2[-1] \oplus [-12] \oplus \bU\) \\
 \(6\) & \(31\) & \(14\) & \([-1] \oplus [-2] \oplus \bU \oplus [2, 1, -3]\) \\
 \(6\) & \(32\) & \(14\) & \(2 [-1] \oplus [-2] \oplus [7] \oplus \bU\) \\
 \(6\) & \(33\) & \(15\) & \([1] \oplus 2[-1] \oplus [-15] \oplus \bU\) \\
 \(6\) & \(34\) & \(15\) & \([-1] \oplus [-3] \oplus \bU \oplus [1, 2, -1]\) \\
 \(6\) & \(35\) & \(16\) & \([1] \oplus [-1] \oplus 2 [-2] \oplus \bU(2)\) \\
 \(6\) & \(36\) & \(16\) & \([-4] \oplus \bU \oplus [0, 2, -1, 0, 1, 1](-1)\) \\
 \(6\) & \(37\) & \(16\) & \([-1] \oplus [-4] \oplus \bU \oplus \bU(2)\) \\
 \(6\) & \(38\) & \(16\) & \([-1] \oplus \bU(2) \oplus [0, 2, -2, 0, 1, 1](-1)\) \\
 \(6\) & \(39\) & \(16\) & \(2 [-1] \oplus [2] \oplus [-8] \oplus \bU\) \\
 \(6\) & \(40\) & \(16\) & \([1] \oplus \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(6\) & \(41\) & \(16\) & \([1] \oplus [-1] \oplus 2 [-4] \oplus \bU\) \\
 \(6\) & \(42\) & \(16\) & \(2 [-1] \oplus \bU \oplus \bU(4)\) \\
 \(6\) & \(43\) & \(16\) & \(2 \bU \oplus [4, 2, 5](-1)\) \\
 \(6\) & \(44\) & \(17\) & \(2 [-1] \oplus \bU \oplus [-2, 1, 8]\) \\
 \(6\) & \(45\) & \(18\) & \(2 [-1] \oplus [1] \oplus [-2] \oplus [3] \oplus [-3]\) \\
 \(6\) & \(46\) & \(20\) & \(2 [-1] \oplus [2] \oplus [-10] \oplus \bU\) \\
 \(6\) & \(47\) & \(20\) & \([1] \oplus [-1] \oplus \bU \oplus [3, 1, 7](-1)\) \\
 \(6\) & \(48\) & \(20\) & \(2 [-1] \oplus [-4] \oplus [5] \oplus \bU\) \\
 \(6\) & \(49\) & \(23\) & \([1] \oplus 2[-1] \oplus [-23] \oplus \bU\) \\
 \(6\) & \(50\) & \(24\) & \([1] \oplus 2[-1] \oplus [-2] \oplus [2, 1, -1](2)\) \\
 \(6\) & \(51\) & \(24\) & \([1] \oplus [-1] \oplus \bU \oplus [4, 2, 7](-1)\) \\
 \(6\) & \(52\) & \(24\) & \(2 [-1] \oplus [-3] \oplus [8] \oplus \bU\) \\
 \(6\) & \(53\) & \(26\) & \(2 [-1] \oplus [-2] \oplus [13] \oplus \bU\) \\
 \(6\) & \(54\) & \(27\) & \([-1] \oplus [-3] \oplus \bU \oplus [-2, 1, 4]\) \\
 \(6\) & \(55\) & \(27\) & \(2[1] \oplus [-1] \oplus 3 [-3] \) \\
 \(6\) & \(56\) & \(27\) & \([1] \oplus [-1] \oplus [0, 3, 2] \oplus \bA_{2}\) \\
 \(6\) & \(57\) & \(28\) & \([-1] \oplus \bU \oplus [-1, 3, -1, 2, 0, 4](-1)\) \\
 \(6\) & \(58\) & \(32\) & \([-1] \oplus [-2] \oplus [-4] \oplus [4] \oplus \bU\) \\
 \(6\) & \(59\) & \(32\) & \(\bU(2) \oplus \bU \oplus [3, 1, 3](-1)\) \\
 \(6\) & \(60\) & \(32\) & \([-1] \oplus [4] \oplus \bU \oplus [3, 1, 3](-1)\) \\
 \(6\) & \(61\) & \(32\) & \([1] \oplus [-1] \oplus [-2] \oplus [-16] \oplus \bU\) \\
 \(6\) & \(62\) & \(32\) & \([-1] \oplus [-2] \oplus 2 \bU(2)\) \\
 \(6\) & \(63\) & \(36\) & \([1] \oplus \bU \oplus [4, 2, 4, 1, -1, 4](-1)\) \\
 \(6\) & \(64\) & \(48\) & \([-1] \oplus \bU(2) \oplus [0, 2, -1, 0, 1, 3](-1)\) \\
 \(6\) & \(65\) & \(48\) & \([1] \oplus [-1] \oplus [-3] \oplus [-4] \oplus \bU(2)\) \\
 \(6\) & \(66\) & \(48\) & \([1] \oplus [-1] \oplus \bU \oplus \bA_{2}(4)\) \\
 \(6\) & \(67\) & \(64\) & \([1] \oplus \bU(2) \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(6\) & \(68\) & \(64\) & \([1] \oplus [-1] \oplus 2 [-2] \oplus \bU(4)\) \\
 \(6\) & \(69\) & \(64\) & \([1] \oplus [-1] \oplus 2 [-4] \oplus \bU(2)\) \\
 \(6\) & \(70\) & \(64\) & \([1] \oplus 3 [-4] \oplus \bU\) \\
 \(6\) & \(71\) & \(64\) & \([-4] \oplus \bU(2) \oplus [0, 2, -1, 0, 1, 1](-1)\) \\
 \(6\) & \(72\) & \(128\) & \(2 \bU(2) \oplus [3, 1, 3](-1)\) \\
 \(6\) & \(73\) & \(192\) & \([-4] \oplus \bU(2) \oplus [0, 2, -1, 0, 1, 3](-1)\) \\
 \(6\) & \(74\) & \(243\) & \([1] \oplus [3] \oplus 4 [-3]\) \\
 \(6\) & \(75\) & \(256\) & \([1] \oplus \bU(4) \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(6\) & \(76\) & \(256\) & \([1] \oplus 3 [-4] \oplus \bU(2)\) \\
\midrule
 \(7\) & \(1\) & \(-1\) & \(3 [-1] \oplus 2 \bU\) \\
 \(7\) & \(2\) & \(-2\) & \(2 [-1] \oplus [-2] \oplus 2 \bU\) \\
 \(7\) & \(3\) & \(-3\) & \(2 [-1] \oplus [-3] \oplus 2 \bU\) \\
 \(7\) & \(4\) & \(-3\) & \(2 [-1] \oplus [1] \oplus \bA_{2} \oplus \bU\) \\
 \(7\) & \(5\) & \(-4\) & \(3 [-1] \oplus [2] \oplus [-2] \oplus \bU\) \\
 \(7\) & \(6\) & \(-4\) & \(3 [-1] \oplus \bU(2) \oplus \bU\) \\
 \(7\) & \(7\) & \(-4\) & \([1] \oplus [-1] \oplus \bU \oplus \bA_{3}\) \\
 \(7\) & \(8\) & \(-4\) & \(2 [-1] \oplus [-4] \oplus 2 \bU\) \\
 \(7\) & \(9\) & \(-5\) & \(2 [-1] \oplus [-5] \oplus 2 \bU\) \\
 \(7\) & \(10\) & \(-5\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(7\) & \(11\) & \(-6\) & \([-1] \oplus [-2] \oplus [-3] \oplus 2 \bU\) \\
 \(7\) & \(12\) & \(-6\) & \([1] \oplus [-1] \oplus [-2] \oplus \bA_{2} \oplus \bU\) \\
 \(7\) & \(13\) & \(-7\) & \(2 [-1] \oplus \bU \oplus [1, 1, -2, 0, 1, 2](-1)\) \\
 \(7\) & \(14\) & \(-7\) & \([-1] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
 \(7\) & \(15\) & \(-8\) & \(2 [-1] \oplus [-2] \oplus \bU(2) \oplus \bU\) \\
 \(7\) & \(16\) & \(-8\) & \([-1] \oplus [-2] \oplus [-4] \oplus 2 \bU\) \\
 \(7\) & \(17\) & \(-8\) & \(2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
 \(7\) & \(18\) & \(-8\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
 \(7\) & \(19\) & \(-8\) & \(2 [-1] \oplus [-8] \oplus 2 \bU\) \\
 \(7\) & \(20\) & \(-9\) & \([1] \oplus 2 \bA_{2} \oplus \bU\) \\
 \(7\) & \(21\) & \(-9\) & \(3 [-1] \oplus \bU(3) \oplus \bU\) \\
 \(7\) & \(22\) & \(-9\) & \(3 [-1] \oplus [2, 1, -4] \oplus \bU\) \\
 \(7\) & \(23\) & \(-10\) & \([-2] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(7\) & \(24\) & \(-10\) & \([-1] \oplus [-2] \oplus [-5] \oplus 2 \bU\) \\
 \(7\) & \(25\) & \(-11\) & \(2 [-1] \oplus [-11] \oplus 2 \bU\) \\
 \(7\) & \(26\) & \(-12\) & \(2 [-1] \oplus [-3] \oplus \bU(2) \oplus \bU\) \\
 \(7\) & \(27\) & \(-12\) & \([1] \oplus [-1] \oplus 2 [-2] \oplus [-3] \oplus \bU\) \\
 \(7\) & \(28\) & \(-12\) & \(2 [-1] \oplus [1] \oplus [-2] \oplus [-6] \oplus \bU\) \\
 \(7\) & \(29\) & \(-12\) & \([-1] \oplus \bU \oplus [1, 1, -3, 0, 2, 1, 0, 0, 1, 2](-1)\) \\
 \(7\) & \(30\) & \(-12\) & \([1] \oplus [-1] \oplus \bU \oplus [2, 1, 4, 0, 1, 2](-1)\) \\
 \(7\) & \(31\) & \(-12\) & \([-1] \oplus [1] \oplus \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
 \(7\) & \(32\) & \(-13\) & \(2 [-1] \oplus [-13] \oplus 2 \bU\) \\
 \(7\) & \(33\) & \(-13\) & \(3 [-1] \oplus [-2, 1, 6] \oplus \bU\) \\
 \(7\) & \(34\) & \(-14\) & \([1] \oplus [-1] \oplus [-2] \oplus [2, 1, 4](-1) \oplus \bU\) \\
 \(7\) & \(35\) & \(-15\) & \([-3] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(7\) & \(36\) & \(-15\) & \([-1] \oplus [-3] \oplus [-5] \oplus 2 \bU\) \\
 \(7\) & \(37\) & \(-16\) & \([-1] \oplus 2 [-2] \oplus [0, 2, 1] \oplus \bU\) \\
 \(7\) & \(38\) & \(-16\) & \([1] \oplus [-1] \oplus [-2] \oplus [3, 1, 3](-1) \oplus \bU\) \\
 \(7\) & \(39\) & \(-16\) & \(\bU \oplus [0, 2, -1, 0, 1, 2, 0, 1, 1, 2, 0, 0, 1, 1, 2](-1)\) \\
 \(7\) & \(40\) & \(-16\) & \([-1] \oplus 2 [-4] \oplus 2 \bU\) \\
 \(7\) & \(41\) & \(-16\) & \([-1] \oplus [-4] \oplus \bU \oplus [0, 2, -2, 0, 1, 1](-1)\) \\
 \(7\) & \(42\) & \(-16\) & \(2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(7\) & \(43\) & \(-16\) & \([1] \oplus [-1] \oplus \bU \oplus [2, 1, 2, 1, 1, 6](-1)\) \\
 \(7\) & \(44\) & \(-16\) & \(2 [-1] \oplus [-16] \oplus 2 \bU\) \\
 \(7\) & \(45\) & \(-16\) & \([-1] \oplus 2 [-2] \oplus \bU(2) \oplus \bU\) \\
 \(7\) & \(46\) & \(-17\) & \([-1] \oplus 2 \bU \oplus [3, 1, 6](-1)\) \\
 \(7\) & \(47\) & \(-18\) & \([-2] \oplus \bU \oplus [0, 3, 1, 0, 1, 1, 0, 1, 0, 1](-1)\) \\
 \(7\) & \(48\) & \(-18\) & \([-2] \oplus 2 [-3] \oplus 2 \bU\) \\
 \(7\) & \(49\) & \(-19\) & \(2 [-1] \oplus [-19] \oplus 2 \bU\) \\
 \(7\) & \(50\) & \(-20\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3](-2)\) \\
 \(7\) & \(51\) & \(-20\) & \(2 \bU \oplus [3, 1, 3, 1, 1, 3](-1)\) \\
 \(7\) & \(52\) & \(-20\) & \([2, 1, 3](-1) \oplus \bU \oplus [-2, 1, 1, 1, 0, 1](-1)\) \\
 \(7\) & \(53\) & \(-21\) & \(2 [-1] \oplus [3] \oplus [2, 1, 4](-1) \oplus \bU\) \\
 \(7\) & \(54\) & \(-21\) & \([-1] \oplus [1] \oplus \bU \oplus [3, 1, 3, 0, 1, 3](-1)\) \\
 \(7\) & \(55\) & \(-22\) & \([1] \oplus [-1] \oplus \bU \oplus [2, 1, 2, 1, 0, 8](-1)\) \\
 \(7\) & \(56\) & \(-24\) & \(2 [-1] \oplus [-6] \oplus \bU(2) \oplus \bU\) \\
 \(7\) & \(57\) & \(-24\) & \([-1] \oplus [-2] \oplus [-12] \oplus 2 \bU\) \\
 \(7\) & \(58\) & \(-24\) & \([1] \oplus [-1] \oplus \bU \oplus [2, 1, 4, 1, 0, 4](-1)\) \\
 \(7\) & \(59\) & \(-24\) & \(\bU \oplus [-1, 1, 2, 1, 0, 2, 0, 1, 0, 2, 0, 0, 1, 1, 3](-1)\) \\
 \(7\) & \(60\) & \(-24\) & \([-1] \oplus [-3] \oplus [-8] \oplus 2 \bU\) \\
 \(7\) & \(61\) & \(-25\) & \(\bU \oplus [1, 1, -1, 0, 1, 1, 0, 1, 0, 3, 0, -1, 0, 2, 3](-1)\) \\
 \(7\) & \(62\) & \(-27\) & \(2 [-1] \oplus [-3] \oplus [2, 1, -4] \oplus \bU\) \\
 \(7\) & \(63\) & \(-27\) & \([-1] \oplus [1] \oplus 3 [-3] \oplus \bU\) \\
 \(7\) & \(64\) & \(-27\) & \([-9] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(7\) & \(65\) & \(-28\) & \(2 [-1] \oplus \bU \oplus [3, 1, 3, 0, 2, -2](-1)\) \\
 \(7\) & \(66\) & \(-28\) & \([1] \oplus [-1] \oplus [-4] \oplus [2, 1, 4](-1) \oplus \bU\) \\
 \(7\) & \(67\) & \(-30\) & \([-2] \oplus [2, 1, -1] \oplus [2, 1, 3](-1) \oplus \bU\) \\
 \(7\) & \(68\) & \(-32\) & \(\bU(2) \oplus \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
 \(7\) & \(69\) & \(-32\) & \(2 [-1] \oplus [-2] \oplus \bU(4) \oplus \bU\) \\
 \(7\) & \(70\) & \(-32\) & \([-1] \oplus \bU \oplus [0, 4, 1, 0, 1, 1, 0, 2, 0, 2](-1)\) \\
 \(7\) & \(71\) & \(-32\) & \([-1] \oplus \bU(2) \oplus [3, 1, 3](-1) \oplus \bU\) \\
 \(7\) & \(72\) & \(-32\) & \([-2] \oplus 2 \bU \oplus [4, 2, 5](-1)\) \\
 \(7\) & \(73\) & \(-32\) & \([-4] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
 \(7\) & \(74\) & \(-32\) & \([-1] \oplus [-2] \oplus [-4] \oplus \bU(2) \oplus \bU\) \\
 \(7\) & \(75\) & \(-33\) & \([-1] \oplus [-3] \oplus [-11] \oplus 2 \bU\) \\
 \(7\) & \(76\) & \(-36\) & \([1] \oplus \bU \oplus [2, 1, 4, 1, 0, 4, 0, -1, 1, 2](-1)\) \\
 \(7\) & \(77\) & \(-36\) & \([1] \oplus [-1] \oplus [-12] \oplus \bA_{2} \oplus \bU\) \\
 \(7\) & \(78\) & \(-40\) & \([-1] \oplus 2 \bU \oplus [7, 3, 7](-1)\) \\
 \(7\) & \(79\) & \(-40\) & \([-8] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(7\) & \(80\) & \(-45\) & \([-15] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(7\) & \(81\) & \(-48\) & \([1] \oplus [-1] \oplus [-4] \oplus \bA_{2}(2) \oplus \bU\) \\
 \(7\) & \(82\) & \(-48\) & \([-1] \oplus [1] \oplus \bU \oplus [3, 1, 3, 1, -1, 7](-1)\) \\
 \(7\) & \(83\) & \(-48\) & \(\bU \oplus [0, 2, -1, 0, 1, 2, 0, 1, 0, 2, 0, 1, -1, 1, 4](-1)\) \\
 \(7\) & \(84\) & \(-48\) & \([-1] \oplus [2] \oplus [-2] \oplus \bA_{2}(2) \oplus \bU\) \\
 \(7\) & \(85\) & \(-49\) & \([-7] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
 \(7\) & \(86\) & \(-54\) & \([-1] \oplus [-2] \oplus [9] \oplus \bA_{2} \oplus \bU\) \\
 \(7\) & \(87\) & \(-64\) & \([0, 2, 1] \oplus \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(7\) & \(88\) & \(-64\) & \([1] \oplus \bU \oplus [3, 1, 3, 1, -1, 3, 1, 1, -1, 5](-1)\) \\
 \(7\) & \(89\) & \(-64\) & \([1] \oplus [-1] \oplus 3 [-4] \oplus \bU\) \\
 \(7\) & \(90\) & \(-64\) & \(\bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 3, 0, -1, 1, 3, 2](-1)\) \\
 \(7\) & \(91\) & \(-64\) & \(2 [-1] \oplus \bU \oplus [-3, 1, 5, 1, -3, 5](-1)\) \\
 \(7\) & \(92\) & \(-64\) & \([-1] \oplus [2] \oplus [-2] \oplus 2 [-4] \oplus \bU\) \\
 \(7\) & \(93\) & \(-64\) & \(\bU(2) \oplus \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(7\) & \(94\) & \(-80\) & \(2 \bU \oplus [4, 2, 7, 0, 2, 4](-1)\) \\
 \(7\) & \(95\) & \(-80\) & \(\bU(2) \oplus \bU \oplus [3, 1, 3, 1, 1, 3](-1)\) \\
 \(7\) & \(96\) & \(-81\) & \([-3] \oplus \bU(3) \oplus \bA_{2} \oplus \bU\) \\
 \(7\) & \(97\) & \(-96\) & \(\bU(2) \oplus \bU \oplus [2, 1, 7, 0, 1, 2](-1)\) \\
 \(7\) & \(98\) & \(-128\) & \(\bU(4) \oplus \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
 \(7\) & \(99\) & \(-128\) & \([-4] \oplus \bU(2) \oplus [3, 1, 3](-1) \oplus \bU\) \\
 \(7\) & \(100\) & \(-144\) & \([1] \oplus 2 \bA_{2}(2) \oplus \bU\) \\
 \(7\) & \(101\) & \(-162\) & \([-2] \oplus 2 [-3] \oplus \bU(3) \oplus \bU\) \\
 \(7\) & \(102\) & \(-192\) & \([-4] \oplus [0, 2, 1] \oplus \bA_{2}(2) \oplus \bU\) \\
 \(7\) & \(103\) & \(-243\) & \([-9] \oplus \bU \oplus [-1, 1, 2, -1, 1, 2, 1, -1, 1, 2](-1)\) \\
 \(7\) & \(104\) & \(-256\) & \([1] \oplus [-16] \oplus \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(7\) & \(105\) & \(-256\) & \(\bU \oplus [1, 1, -1, 0, 2, 4, 0, 2, 0, 4, 0, 2, 2, 2, 6](-1)\) \\
 \(7\) & \(106\) & \(-256\) & \([-4] \oplus \bU \oplus [3, 1, 3, -1, 1, -1, 1, -1, 1, 3](-1)\) \\
 \(7\) & \(107\) & \(-1024\) & \(\bU \oplus [4, 2, -1, -2, 1, 7, 0, 2, 2, 4, 0, 2, 2, 0, 4](-1)\) \\
\midrule
 \(8\) & \(1\) & \(1\) & \(4 [-1] \oplus 2 \bU\) \\
 \(8\) & \(2\) & \(2\) & \(3 [-1] \oplus [-2] \oplus 2 \bU\) \\
 \(8\) & \(3\) & \(3\) & \(3 [-1] \oplus [-3] \oplus 2 \bU\) \\
 \(8\) & \(4\) & \(3\) & \(2 [-1] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(5\) & \(4\) & \(2 [-1] \oplus 2 [-2] \oplus 2 \bU\) \\
 \(8\) & \(6\) & \(4\) & \([-1] \oplus 2 \bU \oplus \bA_{3}\) \\
 \(8\) & \(7\) & \(4\) & \(3 [-1] \oplus [-4] \oplus 2 \bU\) \\
 \(8\) & \(8\) & \(5\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(8\) & \(9\) & \(5\) & \(3 [-1] \oplus [-5] \oplus 2 \bU\) \\
 \(8\) & \(10\) & \(6\) & \(2 [-1] \oplus [-2] \oplus [-3] \oplus 2 \bU\) \\
 \(8\) & \(11\) & \(6\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(12\) & \(7\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3](-1)\) \\
 \(8\) & \(13\) & \(7\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
 \(8\) & \(14\) & \(8\) & \(2 [-1] \oplus [-2] \oplus [-4] \oplus 2 \bU\) \\
 \(8\) & \(15\) & \(8\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 3](-1)\) \\
 \(8\) & \(16\) & \(8\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
 \(8\) & \(17\) & \(8\) & \(2 [-1] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
 \(8\) & \(18\) & \(8\) & \([-1] \oplus 3 [-2] \oplus 2 \bU\) \\
 \(8\) & \(19\) & \(9\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(20\) & \(9\) & \(3 [-1] \oplus [-9] \oplus 2 \bU\) \\
 \(8\) & \(21\) & \(9\) & \(2 [-1] \oplus 2 [-3] \oplus 2 \bU\) \\
 \(8\) & \(22\) & \(10\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(8\) & \(23\) & \(10\) & \(2 [-1] \oplus [-2] \oplus [-5] \oplus 2 \bU\) \\
 \(8\) & \(24\) & \(11\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 3, 0, 0, 1, 2](-1)\) \\
 \(8\) & \(25\) & \(12\) & \(2 \bU \oplus [2, 1, 3, 1, 2, 3, 0, 1, 1, 2](-1)\) \\
 \(8\) & \(26\) & \(12\) & \(2 [-1] \oplus [-2] \oplus [-6] \oplus 2 \bU\) \\
 \(8\) & \(27\) & \(12\) & \([-1] \oplus 2 [-2] \oplus [-3] \oplus 2 \bU\) \\
 \(8\) & \(28\) & \(12\) & \(2 [-1] \oplus [-3] \oplus [-4] \oplus 2 \bU\) \\
 \(8\) & \(29\) & \(12\) & \([-3] \oplus 2 \bU \oplus \bA_{3}\) \\
 \(8\) & \(30\) & \(12\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
 \(8\) & \(31\) & \(13\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 7](-1)\) \\
 \(8\) & \(32\) & \(13\) & \(3 [-1] \oplus [-13] \oplus 2 \bU\) \\
 \(8\) & \(33\) & \(14\) & \([-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 1, 3](-1)\) \\
 \(8\) & \(34\) & \(15\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 3, 1, 0, 0, 3](-1)\) \\
 \(8\) & \(35\) & \(15\) & \(2 [-1] \oplus 2 \bU \oplus [4, 1, 4](-1)\) \\
 \(8\) & \(36\) & \(16\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 3, 0, 1, 1, 2](-1)\) \\
 \(8\) & \(37\) & \(16\) & \(2 [-1] \oplus [-2] \oplus [-8] \oplus 2 \bU\) \\
 \(8\) & \(38\) & \(16\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 3](-1)\) \\
 \(8\) & \(39\) & \(16\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 3, 1, 1, 1, 3](-1)\) \\
 \(8\) & \(40\) & \(16\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 1, 1, 5](-1)\) \\
 \(8\) & \(41\) & \(16\) & \([-1] \oplus 2 [-2] \oplus [-4] \oplus 2 \bU\) \\
 \(8\) & \(42\) & \(17\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 0, 4](-1)\) \\
 \(8\) & \(43\) & \(18\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus [2, 1, 5](-1)\) \\
 \(8\) & \(44\) & \(18\) & \([-1] \oplus [-6] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(45\) & \(19\) & \(2 \bU \oplus [2, 1, 3, 1, 0, 3, 0, 1, 0, 2](-1)\) \\
 \(8\) & \(46\) & \(20\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3, 1, 1, 3](-1)\) \\
 \(8\) & \(47\) & \(20\) & \([-1] \oplus 2 [-2] \oplus [-5] \oplus 2 \bU\) \\
 \(8\) & \(48\) & \(20\) & \([-1] \oplus 2 \bU \oplus [2, 1, 6, 0, 1, 2](-1)\) \\
 \(8\) & \(49\) & \(20\) & \([-1] \oplus [-4] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(8\) & \(50\) & \(21\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
 \(8\) & \(51\) & \(21\) & \(3 [-1] \oplus [-21] \oplus 2 \bU\) \\
 \(8\) & \(52\) & \(22\) & \(2 [-1] \oplus [-2] \oplus [-11] \oplus 2 \bU\) \\
 \(8\) & \(53\) & \(24\) & \([-2] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
 \(8\) & \(54\) & \(24\) & \(2 \bU \oplus [2, 1, 3, 1, 0, 3, 0, 1, 1, 3](-1)\) \\
 \(8\) & \(55\) & \(24\) & \([-1] \oplus [-8] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(56\) & \(24\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
 \(8\) & \(57\) & \(24\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus \bA_{2}(2)\) \\
 \(8\) & \(58\) & \(25\) & \([-1] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(8\) & \(59\) & \(27\) & \(2 [-3] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(60\) & \(27\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 3, 1, 0, 1, 3](-1)\) \\
 \(8\) & \(61\) & \(27\) & \(2 \bU \oplus [2, 1, 5](-1) \oplus \bA_{2}\) \\
 \(8\) & \(62\) & \(28\) & \([-1] \oplus 2 [-2] \oplus [-7] \oplus 2 \bU\) \\
 \(8\) & \(63\) & \(28\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 6](-1)\) \\
 \(8\) & \(64\) & \(30\) & \(2 [-1] \oplus [-3] \oplus [-10] \oplus 2 \bU\) \\
 \(8\) & \(65\) & \(32\) & \([-4] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
 \(8\) & \(66\) & \(32\) & \([-1] \oplus [-4] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
 \(8\) & \(67\) & \(32\) & \(2 [-1] \oplus 2 \bU \oplus [3, 1, 3](-2)\) \\
 \(8\) & \(68\) & \(32\) & \(2 [-1] \oplus [-2] \oplus [-16] \oplus 2 \bU\) \\
 \(8\) & \(69\) & \(32\) & \([-1] \oplus [-2] \oplus 2 [-4] \oplus 2 \bU\) \\
 \(8\) & \(70\) & \(32\) & \(2 [-2] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
 \(8\) & \(71\) & \(32\) & \(2 \bU \oplus [3, 1, 3, -1, 1, 3, -1, 1, 1, 3](-1)\) \\
 \(8\) & \(72\) & \(33\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 1, 9](-1)\) \\
 \(8\) & \(73\) & \(33\) & \([-1] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 5](-1)\) \\
 \(8\) & \(74\) & \(35\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 7, 0, 0, 1, 2](-1)\) \\
 \(8\) & \(75\) & \(36\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus \bA_{2}(2)\) \\
 \(8\) & \(76\) & \(36\) & \([-1] \oplus 2 \bU \oplus [2, 1, 10, 0, 1, 2](-1)\) \\
 \(8\) & \(77\) & \(36\) & \([-3] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 2](-1)\) \\
 \(8\) & \(78\) & \(40\) & \(2 \bU \oplus [2, 1, 3](-1) \oplus [3, 1, 3](-1)\) \\
 \(8\) & \(79\) & \(40\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 6](-1)\) \\
 \(8\) & \(80\) & \(42\) & \([-2] \oplus [-7] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(81\) & \(44\) & \(2 \bU \oplus [2, 1, 3, 0, 1, 2, 0, 1, 0, 6](-1)\) \\
 \(8\) & \(82\) & \(45\) & \([-1] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 5](-1)\) \\
 \(8\) & \(83\) & \(48\) & \([-3] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 3](-1)\) \\
 \(8\) & \(84\) & \(48\) & \(2 \bU \oplus [3, 1, 3, 1, -1, 3, 1, 1, -1, 4](-1)\) \\
 \(8\) & \(85\) & \(48\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 7, 0, 1, 1, 2](-1)\) \\
 \(8\) & \(86\) & \(48\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 5, 1, 1, -1, 5](-1)\) \\
 \(8\) & \(87\) & \(48\) & \([-1] \oplus 2 [-2] \oplus [-12] \oplus 2 \bU\) \\
 \(8\) & \(88\) & \(48\) & \(2 \bU \oplus [3, 1, 3, 1, 1, 3, 1, 1, 1, 3](-1)\) \\
 \(8\) & \(89\) & \(51\) & \(2 \bU \oplus [2, 1, 3, 0, 1, 6, 0, 0, 1, 2](-1)\) \\
 \(8\) & \(90\) & \(54\) & \([-2] \oplus 3 [-3] \oplus 2 \bU\) \\
 \(8\) & \(91\) & \(56\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 4, 1, 0, 1, 4](-1)\) \\
 \(8\) & \(92\) & \(60\) & \([-1] \oplus 2 [-2] \oplus [-15] \oplus 2 \bU\) \\
 \(8\) & \(93\) & \(64\) & \([-8] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
 \(8\) & \(94\) & \(64\) & \(2 [-2] \oplus 2 \bU \oplus [4, 2, 5](-1)\) \\
 \(8\) & \(95\) & \(64\) & \([-4] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 3](-1)\) \\
 \(8\) & \(96\) & \(72\) & \(2 \bU \oplus [2, 1, 6, 0, 1, 3, 0, 1, -1, 3](-1)\) \\
 \(8\) & \(97\) & \(80\) & \(2 \bU \oplus [2, 1, 7, 0, 1, 2, 0, 2, 0, 4](-1)\) \\
 \(8\) & \(98\) & \(80\) & \([-4] \oplus 2 \bU \oplus [3, 1, 3, 1, 1, 3](-1)\) \\
 \(8\) & \(99\) & \(81\) & \([-3] \oplus [-9] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(100\) & \(81\) & \(2 [-3] \oplus 2 \bU \oplus [2, 1, 5](-1)\) \\
 \(8\) & \(101\) & \(96\) & \([-4] \oplus 2 \bU \oplus [2, 1, 7, 0, 1, 2](-1)\) \\
 \(8\) & \(102\) & \(96\) & \(2 \bU \oplus [3, 1, 3](-1) \oplus \bA_{2}(2)\) \\
 \(8\) & \(103\) & \(108\) & \(2 \bU \oplus [2, 1, 7, 0, 1, 2, 0, 3, 0, 6](-1)\) \\
 \(8\) & \(104\) & \(108\) & \([-2] \oplus 2 [-3] \oplus [-6] \oplus 2 \bU\) \\
 \(8\) & \(105\) & \(112\) & \([-7] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(8\) & \(106\) & \(125\) & \([-1] \oplus 3 [-5] \oplus 2 \bU\) \\
 \(8\) & \(107\) & \(128\) & \(2 \bU \oplus [2, 1, 7, -1, 2, 7, 0, 1, 1, 2](-1)\) \\
 \(8\) & \(108\) & \(128\) & \([-2] \oplus 2 \bU \oplus [4, 2, 5, 2, 1, 5](-1)\) \\
 \(8\) & \(109\) & \(128\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 3](-2)\) \\
 \(8\) & \(110\) & \(128\) & \(2 [-4] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
 \(8\) & \(111\) & \(135\) & \(2 \bU \oplus \bA_{2} \oplus [2, 1, 3](-3)\) \\
 \(8\) & \(112\) & \(144\) & \([-3] \oplus [-4] \oplus 2 \bU \oplus \bA_{2}(2)\) \\
 \(8\) & \(113\) & \(162\) & \([-6] \oplus [-9] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(8\) & \(114\) & \(192\) & \([-1] \oplus 2 \bU \oplus [2, 1, 7, 0, 1, 2](-2)\) \\
 \(8\) & \(115\) & \(192\) & \([-3] \oplus 3 [-4] \oplus 2 \bU\) \\
 \(8\) & \(116\) & \(216\) & \(2 \bU \oplus \bA_{2} \oplus [3, 1, 3](-3)\) \\
 \(8\) & \(117\) & \(240\) & \([-15] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(8\) & \(118\) & \(243\) & \(2 \bU \oplus [2, 1, 5](-1) \oplus \bA_{2}(-3)\) \\
 \(8\) & \(119\) & \(256\) & \(2 \bU \oplus [4, 2, 7, 0, 2, 4, 0, 2, 0, 4](-1)\) \\
 \(8\) & \(120\) & \(432\) & \(2 [-3] \oplus 2 \bU \oplus \bA_{2}(-4)\) \\
 \(8\) & \(121\) & \(512\) & \(2 \bU \oplus [4, 2, 7, 2, 3, 7, 2, 3, -1, 7](-1)\) \\
 \(8\) & \(122\) & \(768\) & \(2 \bU \oplus [4, 2, 15, 0, 2, 4, 0, 2, 0, 4](-1)\) \\
\midrule
 \(9\) & \(1\) & \(-1\) & \(5 [-1] \oplus 2 \bU\) \\
 \(9\) & \(2\) & \(-2\) & \(4 [-1] \oplus [-2] \oplus 2 \bU\) \\
 \(9\) & \(3\) & \(-3\) & \(4 [-1] \oplus [-3] \oplus 2 \bU\) \\
 \(9\) & \(4\) & \(-3\) & \(3 [-1] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(9\) & \(5\) & \(-4\) & \(2 [-1] \oplus 2 \bU \oplus \bA_{3}\) \\
 \(9\) & \(6\) & \(-4\) & \(3 [-1] \oplus 2 [-2] \oplus 2 \bU\) \\
 \(9\) & \(7\) & \(-5\) & \(3 [-1] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(9\) & \(8\) & \(-5\) & \(4 [-1] \oplus [-5] \oplus 2 \bU\) \\
 \(9\) & \(9\) & \(-6\) & \(3 [-1] \oplus [-2] \oplus [-3] \oplus 2 \bU\) \\
 \(9\) & \(10\) & \(-6\) & \(4 [-1] \oplus [-6] \oplus 2 \bU\) \\
 \(9\) & \(11\) & \(-7\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3](-1)\) \\
 \(9\) & \(12\) & \(-8\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 0, 0, 3](-1)\) \\
 \(9\) & \(13\) & \(-8\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
 \(9\) & \(14\) & \(-8\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus \bA_{3}\) \\
 \(9\) & \(15\) & \(-9\) & \(4 [-1] \oplus [-9] \oplus 2 \bU\) \\
 \(9\) & \(16\) & \(-9\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 1, 2, 1, 1, 0, 0, 3](-1)\) \\
 \(9\) & \(17\) & \(-9\) & \([-1] \oplus 2 \bU \oplus 2 \bA_{2}\) \\
 \(9\) & \(18\) & \(-10\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 4](-1)\) \\
 \(9\) & \(19\) & \(-11\) & \(4 [-1] \oplus [-11] \oplus 2 \bU\) \\
 \(9\) & \(20\) & \(-11\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3, 0, 0, 1, 2](-1)\) \\
 \(9\) & \(21\) & \(-12\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 3, 0, 0, 0, 1, 2](-1)\) \\
 \(9\) & \(22\) & \(-12\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
 \(9\) & \(23\) & \(-12\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3, 0, 1, -1, 2](-1)\) \\
 \(9\) & \(24\) & \(-12\) & \(2 [-1] \oplus 2 [-2] \oplus [-3] \oplus 2 \bU\) \\
 \(9\) & \(25\) & \(-14\) & \(2 [-1] \oplus [-2] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
 \(9\) & \(26\) & \(-14\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3](-1)\) \\
 \(9\) & \(27\) & \(-15\) & \(2 [-1] \oplus [-5] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(9\) & \(28\) & \(-15\) & \(2 [-1] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(9\) & \(29\) & \(-16\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 3, 1, 1, 1, 3, 0, 0, 1, -1, 2](-1)\) \\
 \(9\) & \(30\) & \(-16\) & \([-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 1, 1, 3](-1)\) \\
 \(9\) & \(31\) & \(-16\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3, 0, 1, 1, 2](-1)\) \\
 \(9\) & \(32\) & \(-17\) & \(4 [-1] \oplus [-17] \oplus 2 \bU\) \\
 \(9\) & \(33\) & \(-18\) & \(3 [-1] \oplus [-3] \oplus [-6] \oplus 2 \bU\) \\
 \(9\) & \(34\) & \(-20\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 6, 0, 1, 2](-1)\) \\
 \(9\) & \(35\) & \(-20\) & \(2 [-1] \oplus [-4] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(9\) & \(36\) & \(-20\) & \([-1] \oplus 2 [-2] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(9\) & \(37\) & \(-21\) & \(2 [-1] \oplus [-7] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(9\) & \(38\) & \(-23\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 5](-1)\) \\
 \(9\) & \(39\) & \(-24\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 3, 1, 0, 1, 0, 4](-1)\) \\
 \(9\) & \(40\) & \(-24\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 0, 0, 7](-1)\) \\
 \(9\) & \(41\) & \(-24\) & \(2 [-1] \oplus [-3] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
 \(9\) & \(42\) & \(-24\) & \(2 [-1] \oplus [-2] \oplus [-3] \oplus [-4] \oplus 2 \bU\) \\
 \(9\) & \(43\) & \(-25\) & \(3 [-1] \oplus 2 [-5] \oplus 2 \bU\) \\
 \(9\) & \(44\) & \(-26\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 4](-1)\) \\
 \(9\) & \(45\) & \(-27\) & \(3 [-1] \oplus [-3] \oplus [-9] \oplus 2 \bU\) \\
 \(9\) & \(46\) & \(-27\) & \([-1] \oplus 2 \bU \oplus \bA_{2} \oplus [2, 1, 5](-1)\) \\
 \(9\) & \(47\) & \(-28\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3, 1, 0, 0, 3](-1)\) \\
 \(9\) & \(48\) & \(-29\) & \(4 [-1] \oplus [-29] \oplus 2 \bU\) \\
 \(9\) & \(49\) & \(-30\) & \(2 [-1] \oplus [-6] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(9\) & \(50\) & \(-32\) & \([-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3, 1, 0, 1, 3](-1)\) \\
 \(9\) & \(51\) & \(-32\) & \([-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 1, 1, 5](-1)\) \\
 \(9\) & \(52\) & \(-32\) & \(2 \bU \oplus [2, 1, 3, 1, 0, 3, 1, 2, 1, 4, 0, 1, -1, 1, 2](-1)\) \\
 \(9\) & \(53\) & \(-35\) & \(2 [-1] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
 \(9\) & \(54\) & \(-36\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 3, 1, 0, 1, 4, 0, 0, 1, 0, 2](-1)\) \\
 \(9\) & \(55\) & \(-36\) & \(2 [-1] \oplus 2 [-3] \oplus [-4] \oplus 2 \bU\) \\
 \(9\) & \(56\) & \(-36\) & \([-1] \oplus 2 [-2] \oplus 2 [-3] \oplus 2 \bU\) \\
 \(9\) & \(57\) & \(-39\) & \(2 [-1] \oplus [-13] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(9\) & \(58\) & \(-40\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 14](-1)\) \\
 \(9\) & \(59\) & \(-41\) & \(4 [-1] \oplus [-41] \oplus 2 \bU\) \\
 \(9\) & \(60\) & \(-44\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 1, 3, 1, 0, 0, 7](-1)\) \\
 \(9\) & \(61\) & \(-44\) & \(2 [-1] \oplus 2 [-2] \oplus [-11] \oplus 2 \bU\) \\
 \(9\) & \(62\) & \(-45\) & \(3 [-1] \oplus 2 \bU \oplus [2, 1, 3](-3)\) \\
 \(9\) & \(63\) & \(-48\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 3, 0, 0, 1, 2, 0, 0, 0, 1, 5](-1)\) \\
 \(9\) & \(64\) & \(-48\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(9\) & \(65\) & \(-48\) & \([-1] \oplus [-4] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
 \(9\) & \(66\) & \(-50\) & \(2 \bU \oplus [2, 1, 3](-1) \oplus [2, 1, 2, 1, 0, 4](-1)\) \\
 \(9\) & \(67\) & \(-54\) & \([-1] \oplus [-2] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 5](-1)\) \\
 \(9\) & \(68\) & \(-54\) & \(3 [-1] \oplus [-6] \oplus [-9] \oplus 2 \bU\) \\
 \(9\) & \(69\) & \(-56\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 3, 1, 0, 0, 3, 0, -1, 1, 0, 3](-1)\) \\
 \(9\) & \(70\) & \(-56\) & \(2 \bU \oplus [2, 1, 4](-1) \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
 \(9\) & \(71\) & \(-60\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3](-1) \oplus \bA_{2}(2)\) \\
 \(9\) & \(72\) & \(-63\) & \([-7] \oplus 2 \bU \oplus 2 \bA_{2}\) \\
 \(9\) & \(73\) & \(-64\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 4, 1, 1, 2, 4, 0, 1, 1, 1, 2](-1)\) \\
 \(9\) & \(74\) & \(-65\) & \(3 [-1] \oplus 2 \bU \oplus [2, 1, 33](-1)\) \\
 \(9\) & \(75\) & \(-72\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 3, 1, 0, 1, 3, 1, 1, 0, 1, 6](-1)\) \\
 \(9\) & \(76\) & \(-75\) & \([-5] \oplus 2 \bU \oplus [2, 1, 3](-1) \oplus \bA_{2}\) \\
 \(9\) & \(77\) & \(-80\) & \([-2] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 3, 0, -1, 1, 3](-1)\) \\
 \(9\) & \(78\) & \(-80\) & \([-1] \oplus 2 [-4] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(9\) & \(79\) & \(-81\) & \([-9] \oplus 2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 1, 3](-1)\) \\
 \(9\) & \(80\) & \(-84\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 8, 0, 1, 0, 2, 0, 1, 1, 0, 2](-1)\) \\
 \(9\) & \(81\) & \(-90\) & \([-1] \oplus [-2] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 8](-1)\) \\
 \(9\) & \(82\) & \(-96\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 5](-1)\) \\
 \(9\) & \(83\) & \(-96\) & \([-2] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 3, 0, 1, 1, 3](-1)\) \\
 \(9\) & \(84\) & \(-96\) & \(2 \bU \oplus [3, 1, 3](-1) \oplus [2, 1, 4, 0, 1, 2](-1)\) \\
 \(9\) & \(85\) & \(-104\) & \(2 \bU \oplus [2, 1, 4, 0, 1, 5, 0, 0, 1, 2, 0, 0, 1, 0, 2](-1)\) \\
 \(9\) & \(86\) & \(-108\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 7, 1, 1, 0, -2, 7](-1)\) \\
 \(9\) & \(87\) & \(-108\) & \(2 [-1] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 5](-2)\) \\
 \(9\) & \(88\) & \(-117\) & \([-1] \oplus 2 \bU \oplus [2, 1, 20](-1) \oplus \bA_{2}\) \\
 \(9\) & \(89\) & \(-120\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3](-1) \oplus [4, 2, 7](-1)\) \\
 \(9\) & \(90\) & \(-125\) & \([-1] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 5, 0, 1, 3](-1)\) \\
 \(9\) & \(91\) & \(-128\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 3, 1, 1, 1, 4, 1, 0, 0, 1, 4](-1)\) \\
 \(9\) & \(92\) & \(-135\) & \(2 \bU \oplus \bA_{2} \oplus [2, 1, 5, 1, 2, 6](-1)\) \\
 \(9\) & \(93\) & \(-140\) & \(2 [-2] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
 \(9\) & \(94\) & \(-144\) & \([-1] \oplus [-6] \oplus [-8] \oplus 2 \bU \oplus \bA_{2}\) \\
 \(9\) & \(95\) & \(-144\) & \([-1] \oplus 2 [-3] \oplus 2 [-4] \oplus 2 \bU\) \\
 \(9\) & \(96\) & \(-176\) & \([-1] \oplus [-11] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
 \(9\) & \(97\) & \(-189\) & \([-7] \oplus 2 \bU \oplus [2, 1, 5](-1) \oplus \bA_{2}\) \\
 \(9\) & \(98\) & \(-192\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 4, -1, 0, 1, 4, 0, 0, 1, -1, 5](-1)\) \\
 \(9\) & \(99\) & \(-200\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 7, 1, 1, 2, 7, 0, 0, 1, 1, 2](-1)\) \\
 \(9\) & \(100\) & \(-216\) & \(2 \bU \oplus [2, 1, 6, 0, 1, 3, 0, 1, -1, 3, 0, 1, 1, 1, 4](-1)\) \\
 \(9\) & \(101\) & \(-216\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 3, 1, 0, 0, 6, 1, 0, 1, -2, 8](-1)\) \\
 \(9\) & \(102\) & \(-300\) & \([-2] \oplus [-5] \oplus [-6] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
 \(9\) & \(103\) & \(-320\) & \(2 \bU \oplus [2, 1, 4, 1, 2, 4, 0, -1, 1, 5, 0, -1, 1, 1, 5](-1)\) \\
 \(9\) & \(104\) & \(-360\) & \([-3] \oplus 2 \bU \oplus [2, 1, 8](-1) \oplus [3, 1, 3](-1)\) \\
 \(9\) & \(105\) & \(-384\) & \(2 \bU \oplus [3, 1, 3, -1, 1, 6, 0, 0, 1, 4, 0, 0, 2, 2, 4](-1)\) \\
 \(9\) & \(106\) & \(-432\) & \([-3] \oplus 2 \bU \oplus [3, 1, 4, 1, 0, 4, 1, 0, 0, 4](-1)\) \\
 \(9\) & \(107\) & \(-441\) & \([-21] \oplus 2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 0, 0, 6](-1)\) \\
 \(9\) & \(108\) & \(-560\) & \(2 \bU \oplus [2, 1, 4](-1) \oplus [4, 2, 7, 0, 2, 4](-1)\) \\
 \(9\) & \(109\) & \(-576\) & \([-1] \oplus 2 \bU \oplus [6, 3, 7, -3, 1, 7, 3, 0, 0, 7](-1)\) \\
 \(9\) & \(110\) & \(-1200\) & \(2 \bU \oplus [3, 1, 4, 1, 0, 4, 1, 2, 2, 7, 1, 2, 2, 2, 8](-1)\) \\
\midrule
 \(10\) & \(1\) & \(1\) & \(2 [1] \oplus \bE_{8}\) \\
 \(10\) & \(2\) & \(2\) & \([1] \oplus [2] \oplus \bE_{8}\) \\
 \(10\) & \(3\) & \(3\) & \([1] \oplus [3] \oplus \bE_{8}\) \\
 \(10\) & \(4\) & \(4\) & \([1] \oplus [4] \oplus \bE_{8}\) \\
 \(10\) & \(5\) & \(5\) & \([1] \oplus [5] \oplus \bE_{8}\) \\
 \(10\) & \(6\) & \(6\) & \([1] \oplus [6] \oplus \bE_{8}\) \\
 \(10\) & \(7\) & \(7\) & \([1] \oplus [7] \oplus \bE_{8}\) \\
 \(10\) & \(8\) & \(8\) & \([1] \oplus [8] \oplus \bE_{8}\) \\
 \(10\) & \(9\) & \(9\) & \([1] \oplus [9] \oplus \bE_{8}\) \\
 \(10\) & \(10\) & \(10\) & \([1] \oplus [10] \oplus \bE_{8}\) \\
 \(10\) & \(11\) & \(12\) & \([1] \oplus [12] \oplus \bE_{8}\) \\
 \(10\) & \(12\) & \(13\) & \([1] \oplus [13] \oplus \bE_{8}\) \\
 \(10\) & \(13\) & \(15\) & \([1] \oplus [15] \oplus \bE_{8}\) \\
 \(10\) & \(14\) & \(16\) & \([1] \oplus [16] \oplus \bE_{8}\) \\
 \(10\) & \(15\) & \(18\) & \([1] \oplus [18] \oplus \bE_{8}\) \\
 \(10\) & \(16\) & \(21\) & \([1] \oplus [21] \oplus \bE_{8}\) \\
 \(10\) & \(17\) & \(22\) & \([1] \oplus [22] \oplus \bE_{8}\) \\
 \(10\) & \(18\) & \(24\) & \([1] \oplus [24] \oplus \bE_{8}\) \\
 \(10\) & \(19\) & \(25\) & \([1] \oplus [25] \oplus \bE_{8}\) \\
 \(10\) & \(20\) & \(28\) & \([1] \oplus [28] \oplus \bE_{8}\) \\
 \(10\) & \(21\) & \(30\) & \([1] \oplus [30] \oplus \bE_{8}\) \\
 \(10\) & \(22\) & \(33\) & \([1] \oplus [33] \oplus \bE_{8}\) \\
 \(10\) & \(23\) & \(37\) & \([1] \oplus [37] \oplus \bE_{8}\) \\
 \(10\) & \(24\) & \(40\) & \([1] \oplus [40] \oplus \bE_{8}\) \\
 \(10\) & \(25\) & \(42\) & \([1] \oplus [42] \oplus \bE_{8}\) \\
 \(10\) & \(26\) & \(45\) & \([1] \oplus [45] \oplus \bE_{8}\) \\
 \(10\) & \(27\) & \(48\) & \([1] \oplus [48] \oplus \bE_{8}\) \\
 \(10\) & \(28\) & \(57\) & \([1] \oplus [57] \oplus \bE_{8}\) \\
 \(10\) & \(29\) & \(58\) & \([1] \oplus [58] \oplus \bE_{8}\) \\
 \(10\) & \(30\) & \(60\) & \([1] \oplus [60] \oplus \bE_{8}\) \\
 \(10\) & \(31\) & \(70\) & \([1] \oplus [70] \oplus \bE_{8}\) \\
 \(10\) & \(32\) & \(72\) & \([1] \oplus [72] \oplus \bE_{8}\) \\
 \(10\) & \(33\) & \(78\) & \([1] \oplus [78] \oplus \bE_{8}\) \\
 \(10\) & \(34\) & \(85\) & \([1] \oplus [85] \oplus \bE_{8}\) \\
 \(10\) & \(35\) & \(88\) & \([1] \oplus [88] \oplus \bE_{8}\) \\
 \(10\) & \(36\) & \(93\) & \([1] \oplus [93] \oplus \bE_{8}\) \\
 \(10\) & \(37\) & \(102\) & \([1] \oplus [102] \oplus \bE_{8}\) \\
 \(10\) & \(38\) & \(105\) & \([1] \oplus [105] \oplus \bE_{8}\) \\
 \(10\) & \(39\) & \(112\) & \([1] \oplus [112] \oplus \bE_{8}\) \\
 \(10\) & \(40\) & \(120\) & \([1] \oplus [120] \oplus \bE_{8}\) \\
 \(10\) & \(41\) & \(130\) & \([1] \oplus [130] \oplus \bE_{8}\) \\
 \(10\) & \(42\) & \(133\) & \([1] \oplus [133] \oplus \bE_{8}\) \\
 \(10\) & \(43\) & \(165\) & \([1] \oplus [165] \oplus \bE_{8}\) \\
 \(10\) & \(44\) & \(168\) & \([1] \oplus [168] \oplus \bE_{8}\) \\
 \(10\) & \(45\) & \(177\) & \([1] \oplus [177] \oplus \bE_{8}\) \\
 \(10\) & \(46\) & \(190\) & \([1] \oplus [190] \oplus \bE_{8}\) \\
 \(10\) & \(47\) & \(210\) & \([1] \oplus [210] \oplus \bE_{8}\) \\
 \(10\) & \(48\) & \(232\) & \([1] \oplus [232] \oplus \bE_{8}\) \\
 \(10\) & \(49\) & \(240\) & \([1] \oplus [240] \oplus \bE_{8}\) \\
 \(10\) & \(50\) & \(253\) & \([1] \oplus [253] \oplus \bE_{8}\) \\
 \(10\) & \(51\) & \(273\) & \([1] \oplus [273] \oplus \bE_{8}\) \\
 \(10\) & \(52\) & \(280\) & \([1] \oplus [280] \oplus \bE_{8}\) \\
 \(10\) & \(53\) & \(312\) & \([1] \oplus [312] \oplus \bE_{8}\) \\
 \(10\) & \(54\) & \(330\) & \([1] \oplus [330] \oplus \bE_{8}\) \\
 \(10\) & \(55\) & \(345\) & \([1] \oplus [345] \oplus \bE_{8}\) \\
 \(10\) & \(56\) & \(357\) & \([1] \oplus [357] \oplus \bE_{8}\) \\
 \(10\) & \(57\) & \(385\) & \([1] \oplus [385] \oplus \bE_{8}\) \\
 \(10\) & \(58\) & \(408\) & \([1] \oplus [408] \oplus \bE_{8}\) \\
 \(10\) & \(59\) & \(462\) & \([1] \oplus [462] \oplus \bE_{8}\) \\
 \(10\) & \(60\) & \(520\) & \([1] \oplus [520] \oplus \bE_{8}\) \\
 \(10\) & \(61\) & \(760\) & \([1] \oplus [760] \oplus \bE_{8}\) \\
 \(10\) & \(62\) & \(840\) & \([1] \oplus [840] \oplus \bE_{8}\) \\
 \(10\) & \(63\) & \(1320\) & \([1] \oplus [1320] \oplus \bE_{8}\) \\
 \(10\) & \(64\) & \(1365\) & \([1] \oplus [1365] \oplus \bE_{8}\) \\
 \(10\) & \(65\) & \(1848\) & \([1] \oplus [1848] \oplus \bE_{8}\) \\
\midrule
 \(11\) & \(1\) & \(-1\) & \([1] \oplus \bU \oplus \bE_{8}\) \\


\end{longtable}

\end{center}


==> tabs/half_co-id_short.tex <==
\begin{center}
\renewcommand{\arraystretch}{1.2}
%\small
%\scriptsize
\footnotesize

\begin{longtable}{llll}
  \caption{Halves of co-idoneal lattices of rank \(\lambda\leq 5\) (see \autoref{thm:co-idoneal}). For the complete list, see the ancillary file \texttt{half.co-idoneal.lat.txt} on arXiv.}
  \label{tab:half_co-id} \\
  
    \toprule
        $\lambda$ & No. & $\det T'$ & $T'$ \\
    \midrule
  \endfirsthead

    \multicolumn{4}{c}%
    {\tablename\ \thetable{}, continued from previous page.} \\
    \midrule
        $\lambda$ & No. & $\det T'$ & $T'$ \\
    \midrule
  \endhead

    \multicolumn{4}{c}{Continued on next page.} \\ \midrule
  \endfoot

    \bottomrule
  \endlastfoot

 \(2\) & \(1\) & \(1\) & \(2 [1]\) \\
 \(2\) & \(2\) & \(2\) & \([1] \oplus [2]\) \\
 \(2\) & \(3\) & \(4\) & \([1] \oplus [4]\) \\
\midrule
 \(3\) & \(1\) & \(-1\) & \([1] \oplus \bU\) \\
 \(3\) & \(2\) & \(-2\) & \([1] \oplus [2] \oplus [-1]\) \\
 \(3\) & \(3\) & \(-3\) & \(2 [1] \oplus [-3]\) \\
 \(3\) & \(4\) & \(-4\) & \([1] \oplus [2] \oplus [-2]\) \\
 \(3\) & \(5\) & \(-4\) & \([1] \oplus \bU(2)\) \\
 \(3\) & \(6\) & \(-5\) & \([1] \oplus [2, 1, -2]\) \\
 \(3\) & \(7\) & \(-8\) & \([2] \oplus [0, 2, -1]\) \\
 \(3\) & \(8\) & \(-9\) & \([-1] \oplus 2 [3]\) \\
\midrule
 \(4\) & \(1\) & \(1\) & \(2 [1] \oplus 2 [-1]\) \\
 \(4\) & \(2\) & \(2\) & \([1] \oplus [-2] \oplus \bU\) \\
 \(4\) & \(3\) & \(3\) & \([-1] \oplus [3] \oplus \bU\) \\
 \(4\) & \(4\) & \(4\) & \([1] \oplus [-1, 1, 1, -1, 1, 1](-1)\) \\
 \(4\) & \(5\) & \(4\) & \([1] \oplus [-1] \oplus \bU(2)\) \\
 \(4\) & \(6\) & \(4\) & \([1] \oplus [-1] \oplus [0, 2, -1]\) \\
 \(4\) & \(7\) & \(4\) & \([1] \oplus [-1] \oplus [0, 2, 1]\) \\
 \(4\) & \(8\) & \(5\) & \([-1] \oplus [1] \oplus [2, 1, -2]\) \\
 \(4\) & \(9\) & \(6\) & \([1] \oplus [1, 2, -1, 0, 1, 1](-1)\) \\
 \(4\) & \(10\) & \(8\) & \([1] \oplus [2] \oplus 2 [-2]\) \\
 \(4\) & \(11\) & \(8\) & \([1] \oplus [-2, 1, 2, 0, 1, 2](-1)\) \\
 \(4\) & \(12\) & \(9\) & \([3] \oplus [-3] \oplus \bU\) \\
 \(4\) & \(13\) & \(9\) & \([0, 3, 2, 0, 2, 0, 0, -5, 1, 1]\) \\
 \(4\) & \(14\) & \(12\) & \([3] \oplus [0, 2, -2, 0, 1, 1](-1)\) \\
 \(4\) & \(15\) & \(16\) & \([-4] \oplus [0, 2, 1, 0, 1, 1]\) \\
 \(4\) & \(16\) & \(16\) & \([4] \oplus [0, 2, 1, 0, 1, 1](-1)\) \\
 \(4\) & \(17\) & \(16\) & \([1] \oplus [-1] \oplus \bU(4)\) \\
\midrule
 \(5\) & \(1\) & \(-1\) & \([-1] \oplus 2 \bU\) \\
 \(5\) & \(2\) & \(-2\) & \([1] \oplus [-1] \oplus [-2] \oplus \bU\) \\
 \(5\) & \(3\) & \(-3\) & \(2 [-1] \oplus [3] \oplus \bU\) \\
 \(5\) & \(4\) & \(-3\) & \([1] \oplus [-1] \oplus [-3] \oplus \bU\) \\
 \(5\) & \(5\) & \(-4\) & \([1] \oplus 2[-1] \oplus [2] \oplus [-2]\) \\
 \(5\) & \(6\) & \(-4\) & \([-1] \oplus \bU \oplus \bU(2)\) \\
 \(5\) & \(7\) & \(-4\) & \([1] \oplus [-1] \oplus [-4] \oplus \bU\) \\
 \(5\) & \(8\) & \(-4\) & \([-1] \oplus \bU \oplus [-1, 1, 3]\) \\
 \(5\) & \(9\) & \(-5\) & \(2 [-1] \oplus [5] \oplus \bU\) \\
 \(5\) & \(10\) & \(-6\) & \([1] \oplus [-1] \oplus [-6] \oplus \bU\) \\
 \(5\) & \(11\) & \(-7\) & \([-1] \oplus \bU \oplus [2, 1, -3]\) \\
 \(5\) & \(12\) & \(-7\) & \(2 [-1] \oplus [7] \oplus \bU\) \\
 \(5\) & \(13\) & \(-8\) & \([1] \oplus [-1] \oplus [-2] \oplus \bU(2)\) \\
 \(5\) & \(14\) & \(-8\) & \([-1] \oplus [-2] \oplus [4] \oplus \bU\) \\
 \(5\) & \(15\) & \(-8\) & \(2 [-1] \oplus [8] \oplus \bU\) \\
 \(5\) & \(16\) & \(-8\) & \([-1] \oplus [1] \oplus [0, 2, -2, 0, 1, 2](-1)\) \\
 \(5\) & \(17\) & \(-8\) & \([1] \oplus [-1] \oplus [-8] \oplus \bU\) \\
 \(5\) & \(18\) & \(-9\) & \(\bU \oplus [0, 3, -2, 0, 1, 1](-1)\) \\
 \(5\) & \(19\) & \(-9\) & \([0, 3, 2, 0, 1, 0, 0, 1, 0, 1, 0, 1, 1, 0, 0](-1)\) \\
 \(5\) & \(20\) & \(-10\) & \([1] \oplus [-1] \oplus [-10] \oplus \bU\) \\
 \(5\) & \(21\) & \(-12\) & \([1] \oplus [-1] \oplus [-3] \oplus \bU(2)\) \\
 \(5\) & \(22\) & \(-12\) & \(2 [-1] \oplus [3] \oplus \bU(2)\) \\
 \(5\) & \(23\) & \(-12\) & \(2[-1] \oplus [1] \oplus [2, 1, -1](2)\) \\
 \(5\) & \(24\) & \(-12\) & \([-1] \oplus [-3] \oplus [4] \oplus \bU\) \\
 \(5\) & \(25\) & \(-13\) & \(2 [-1] \oplus [13] \oplus \bU\) \\
 \(5\) & \(26\) & \(-15\) & \([3] \oplus \bU \oplus [2, 1, 3](-1)\) \\
 \(5\) & \(27\) & \(-16\) & \([-1] \oplus 2 \bU(2)\) \\
 \(5\) & \(28\) & \(-16\) & \([1] \oplus [-1] \oplus [-4] \oplus \bU(2)\) \\
 \(5\) & \(29\) & \(-16\) & \([1] \oplus 2 [-4] \oplus \bU\) \\
 \(5\) & \(30\) & \(-16\) & \([0, 2, -2, 0, 1, 1, 0, 1, 0, -2, 0, 1, 0, 0, 2](-1)\) \\
 \(5\) & \(31\) & \(-16\) & \([-4] \oplus \bU \oplus [-1, 1, 3]\) \\
 \(5\) & \(32\) & \(-16\) & \([1] \oplus [-1] \oplus [-16] \oplus \bU\) \\
 \(5\) & \(33\) & \(-18\) & \([-1] \oplus [-2] \oplus [9] \oplus \bU\) \\
 \(5\) & \(34\) & \(-20\) & \(2 [-1] \oplus [5] \oplus \bU(2)\) \\
 \(5\) & \(35\) & \(-21\) & \([-1] \oplus [-3] \oplus [7] \oplus \bU\) \\
 \(5\) & \(36\) & \(-24\) & \([1] \oplus [-1] \oplus [-24] \oplus \bU\) \\
 \(5\) & \(37\) & \(-27\) & \([1] \oplus [-1] \oplus [3] \oplus 2[-3]\) \\
 \(5\) & \(38\) & \(-32\) & \([1] \oplus [-1] \oplus [-2] \oplus \bU(4)\) \\
 \(5\) & \(39\) & \(-32\) & \([1] \oplus [-1] \oplus [-8] \oplus \bU(2)\) \\
 \(5\) & \(40\) & \(-48\) & \(\bU(2) \oplus [0, 2, -1, 0, 1, 3](-1)\) \\
 \(5\) & \(41\) & \(-64\) & \([1] \oplus 2 [-4] \oplus \bU(2)\) \\
% \midrule
%  \(6\) & \(1\) & \(1\) & \(2 [-1] \oplus 2 \bU\) \\
%  \(6\) & \(2\) & \(2\) & \(2 [-1] \oplus [1] \oplus [-2] \oplus \bU\) \\
%  \(6\) & \(3\) & \(3\) & \([-1] \oplus [-3] \oplus 2 \bU\) \\
%  \(6\) & \(4\) & \(3\) & \([1] \oplus [-1] \oplus \bU \oplus \bA_{2}\) \\
%  \(6\) & \(5\) & \(4\) & \([1] \oplus [-1] \oplus 2 [-2] \oplus \bU\) \\
%  \(6\) & \(6\) & \(4\) & \(2 [-1] \oplus \bU \oplus \bU(2)\) \\
%  \(6\) & \(7\) & \(4\) & \(2 [-1] \oplus \bU \oplus [0, 2, -1]\) \\
%  \(6\) & \(8\) & \(4\) & \([-1] \oplus [-4] \oplus 2 \bU\) \\
%  \(6\) & \(9\) & \(5\) & \(3 [-1] \oplus [5] \oplus \bU\) \\
%  \(6\) & \(10\) & \(5\) & \(2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(6\) & \(11\) & \(6\) & \(2 [-1] \oplus [-2] \oplus [3] \oplus \bU\) \\
%  \(6\) & \(12\) & \(6\) & \([1] \oplus [-1] \oplus [-2] \oplus [-3] \oplus \bU\) \\
%  \(6\) & \(13\) & \(7\) & \([1] \oplus 2[-1] \oplus [-7] \oplus \bU\) \\
%  \(6\) & \(14\) & \(8\) & \([-1] \oplus [-2] \oplus \bU(2) \oplus \bU\) \\
%  \(6\) & \(15\) & \(8\) & \(2 [-1] \oplus [-2] \oplus [4] \oplus \bU\) \\
%  \(6\) & \(16\) & \(8\) & \(3 [-1] \oplus [8] \oplus \bU\) \\
%  \(6\) & \(17\) & \(8\) & \([-1] \oplus [1] \oplus \bU \oplus [3, 1, 3](-1)\) \\
%  \(6\) & \(18\) & \(8\) & \([-1] \oplus [-8] \oplus 2 \bU\) \\
%  \(6\) & \(19\) & \(9\) & \([1] \oplus [-1] \oplus 2 [-3] \oplus \bU\) \\
%  \(6\) & \(20\) & \(9\) & \(2 [-1] \oplus \bU \oplus [-2, 1, 4]\) \\
%  \(6\) & \(21\) & \(9\) & \(3 [-1] \oplus [9] \oplus \bU\) \\
%  \(6\) & \(22\) & \(10\) & \(2 [-1] \oplus [-2] \oplus [5] \oplus \bU\) \\
%  \(6\) & \(23\) & \(11\) & \([-1] \oplus [1] \oplus \bU \oplus [3, 1, 4](-1)\) \\
%  \(6\) & \(24\) & \(11\) & \([1] \oplus [-1] \oplus [-2, 1, 2, 0, 1, 2, 0, 1, 1, 2](-1)\) \\
%  \(6\) & \(25\) & \(12\) & \([1] \oplus [-1] \oplus \bU(2) \oplus \bA_{2}\) \\
%  \(6\) & \(26\) & \(12\) & \([1] \oplus [-1] \oplus [-2] \oplus [-6] \oplus \bU\) \\
%  \(6\) & \(27\) & \(12\) & \([-1] \oplus [-3] \oplus \bU \oplus \bU(2)\) \\
%  \(6\) & \(28\) & \(12\) & \([1] \oplus [-1] \oplus [-3] \oplus [-4] \oplus \bU\) \\
%  \(6\) & \(29\) & \(12\) & \([1] \oplus [-4] \oplus \bU \oplus \bA_{2}\) \\
%  \(6\) & \(30\) & \(12\) & \([1] \oplus 2[-1] \oplus [-12] \oplus \bU\) \\
%  \(6\) & \(31\) & \(14\) & \([-1] \oplus [-2] \oplus \bU \oplus [2, 1, -3]\) \\
%  \(6\) & \(32\) & \(14\) & \(2 [-1] \oplus [-2] \oplus [7] \oplus \bU\) \\
%  \(6\) & \(33\) & \(15\) & \([1] \oplus 2[-1] \oplus [-15] \oplus \bU\) \\
%  \(6\) & \(34\) & \(15\) & \([-1] \oplus [-3] \oplus \bU \oplus [1, 2, -1]\) \\
%  \(6\) & \(35\) & \(16\) & \([1] \oplus [-1] \oplus 2 [-2] \oplus \bU(2)\) \\
%  \(6\) & \(36\) & \(16\) & \([-4] \oplus \bU \oplus [0, 2, -1, 0, 1, 1](-1)\) \\
%  \(6\) & \(37\) & \(16\) & \([-1] \oplus [-4] \oplus \bU \oplus \bU(2)\) \\
%  \(6\) & \(38\) & \(16\) & \([-1] \oplus \bU(2) \oplus [0, 2, -2, 0, 1, 1](-1)\) \\
%  \(6\) & \(39\) & \(16\) & \(2 [-1] \oplus [2] \oplus [-8] \oplus \bU\) \\
%  \(6\) & \(40\) & \(16\) & \([1] \oplus \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(6\) & \(41\) & \(16\) & \([1] \oplus [-1] \oplus 2 [-4] \oplus \bU\) \\
%  \(6\) & \(42\) & \(16\) & \(2 [-1] \oplus \bU \oplus \bU(4)\) \\
%  \(6\) & \(43\) & \(16\) & \(2 \bU \oplus [4, 2, 5](-1)\) \\
%  \(6\) & \(44\) & \(17\) & \(2 [-1] \oplus \bU \oplus [-2, 1, 8]\) \\
%  \(6\) & \(45\) & \(18\) & \(2 [-1] \oplus [1] \oplus [-2] \oplus [3] \oplus [-3]\) \\
%  \(6\) & \(46\) & \(20\) & \(2 [-1] \oplus [2] \oplus [-10] \oplus \bU\) \\
%  \(6\) & \(47\) & \(20\) & \([1] \oplus [-1] \oplus \bU \oplus [3, 1, 7](-1)\) \\
%  \(6\) & \(48\) & \(20\) & \(2 [-1] \oplus [-4] \oplus [5] \oplus \bU\) \\
%  \(6\) & \(49\) & \(23\) & \([1] \oplus 2[-1] \oplus [-23] \oplus \bU\) \\
%  \(6\) & \(50\) & \(24\) & \([1] \oplus 2[-1] \oplus [-2] \oplus [2, 1, -1](2)\) \\
%  \(6\) & \(51\) & \(24\) & \([1] \oplus [-1] \oplus \bU \oplus [4, 2, 7](-1)\) \\
%  \(6\) & \(52\) & \(24\) & \(2 [-1] \oplus [-3] \oplus [8] \oplus \bU\) \\
%  \(6\) & \(53\) & \(26\) & \(2 [-1] \oplus [-2] \oplus [13] \oplus \bU\) \\
%  \(6\) & \(54\) & \(27\) & \([-1] \oplus [-3] \oplus \bU \oplus [-2, 1, 4]\) \\
%  \(6\) & \(55\) & \(27\) & \(2[1] \oplus [-1] \oplus 3 [-3] \) \\
%  \(6\) & \(56\) & \(27\) & \([1] \oplus [-1] \oplus [0, 3, 2] \oplus \bA_{2}\) \\
%  \(6\) & \(57\) & \(28\) & \([-1] \oplus \bU \oplus [-1, 3, -1, 2, 0, 4](-1)\) \\
%  \(6\) & \(58\) & \(32\) & \([-1] \oplus [-2] \oplus [-4] \oplus [4] \oplus \bU\) \\
%  \(6\) & \(59\) & \(32\) & \(\bU(2) \oplus \bU \oplus [3, 1, 3](-1)\) \\
%  \(6\) & \(60\) & \(32\) & \([-1] \oplus [4] \oplus \bU \oplus [3, 1, 3](-1)\) \\
%  \(6\) & \(61\) & \(32\) & \([1] \oplus [-1] \oplus [-2] \oplus [-16] \oplus \bU\) \\
%  \(6\) & \(62\) & \(32\) & \([-1] \oplus [-2] \oplus 2 \bU(2)\) \\
%  \(6\) & \(63\) & \(36\) & \([1] \oplus \bU \oplus [4, 2, 4, 1, -1, 4](-1)\) \\
%  \(6\) & \(64\) & \(48\) & \([-1] \oplus \bU(2) \oplus [0, 2, -1, 0, 1, 3](-1)\) \\
%  \(6\) & \(65\) & \(48\) & \([1] \oplus [-1] \oplus [-3] \oplus [-4] \oplus \bU(2)\) \\
%  \(6\) & \(66\) & \(48\) & \([1] \oplus [-1] \oplus \bU \oplus \bA_{2}(4)\) \\
%  \(6\) & \(67\) & \(64\) & \([1] \oplus \bU(2) \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(6\) & \(68\) & \(64\) & \([1] \oplus [-1] \oplus 2 [-2] \oplus \bU(4)\) \\
%  \(6\) & \(69\) & \(64\) & \([1] \oplus [-1] \oplus 2 [-4] \oplus \bU(2)\) \\
%  \(6\) & \(70\) & \(64\) & \([1] \oplus 3 [-4] \oplus \bU\) \\
%  \(6\) & \(71\) & \(64\) & \([-4] \oplus \bU(2) \oplus [0, 2, -1, 0, 1, 1](-1)\) \\
%  \(6\) & \(72\) & \(128\) & \(2 \bU(2) \oplus [3, 1, 3](-1)\) \\
%  \(6\) & \(73\) & \(192\) & \([-4] \oplus \bU(2) \oplus [0, 2, -1, 0, 1, 3](-1)\) \\
%  \(6\) & \(74\) & \(243\) & \([1] \oplus [3] \oplus 4 [-3]\) \\
%  \(6\) & \(75\) & \(256\) & \([1] \oplus \bU(4) \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(6\) & \(76\) & \(256\) & \([1] \oplus 3 [-4] \oplus \bU(2)\) \\
% \midrule
%  \(7\) & \(1\) & \(-1\) & \(3 [-1] \oplus 2 \bU\) \\
%  \(7\) & \(2\) & \(-2\) & \(2 [-1] \oplus [-2] \oplus 2 \bU\) \\
%  \(7\) & \(3\) & \(-3\) & \(2 [-1] \oplus [-3] \oplus 2 \bU\) \\
%  \(7\) & \(4\) & \(-3\) & \(2 [-1] \oplus [1] \oplus \bA_{2} \oplus \bU\) \\
%  \(7\) & \(5\) & \(-4\) & \(3 [-1] \oplus [2] \oplus [-2] \oplus \bU\) \\
%  \(7\) & \(6\) & \(-4\) & \(3 [-1] \oplus \bU(2) \oplus \bU\) \\
%  \(7\) & \(7\) & \(-4\) & \([1] \oplus [-1] \oplus \bU \oplus \bA_{3}\) \\
%  \(7\) & \(8\) & \(-4\) & \(2 [-1] \oplus [-4] \oplus 2 \bU\) \\
%  \(7\) & \(9\) & \(-5\) & \(2 [-1] \oplus [-5] \oplus 2 \bU\) \\
%  \(7\) & \(10\) & \(-5\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(7\) & \(11\) & \(-6\) & \([-1] \oplus [-2] \oplus [-3] \oplus 2 \bU\) \\
%  \(7\) & \(12\) & \(-6\) & \([1] \oplus [-1] \oplus [-2] \oplus \bA_{2} \oplus \bU\) \\
%  \(7\) & \(13\) & \(-7\) & \(2 [-1] \oplus \bU \oplus [1, 1, -2, 0, 1, 2](-1)\) \\
%  \(7\) & \(14\) & \(-7\) & \([-1] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
%  \(7\) & \(15\) & \(-8\) & \(2 [-1] \oplus [-2] \oplus \bU(2) \oplus \bU\) \\
%  \(7\) & \(16\) & \(-8\) & \([-1] \oplus [-2] \oplus [-4] \oplus 2 \bU\) \\
%  \(7\) & \(17\) & \(-8\) & \(2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
%  \(7\) & \(18\) & \(-8\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
%  \(7\) & \(19\) & \(-8\) & \(2 [-1] \oplus [-8] \oplus 2 \bU\) \\
%  \(7\) & \(20\) & \(-9\) & \([1] \oplus 2 \bA_{2} \oplus \bU\) \\
%  \(7\) & \(21\) & \(-9\) & \(3 [-1] \oplus \bU(3) \oplus \bU\) \\
%  \(7\) & \(22\) & \(-9\) & \(3 [-1] \oplus [2, 1, -4] \oplus \bU\) \\
%  \(7\) & \(23\) & \(-10\) & \([-2] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(7\) & \(24\) & \(-10\) & \([-1] \oplus [-2] \oplus [-5] \oplus 2 \bU\) \\
%  \(7\) & \(25\) & \(-11\) & \(2 [-1] \oplus [-11] \oplus 2 \bU\) \\
%  \(7\) & \(26\) & \(-12\) & \(2 [-1] \oplus [-3] \oplus \bU(2) \oplus \bU\) \\
%  \(7\) & \(27\) & \(-12\) & \([1] \oplus [-1] \oplus 2 [-2] \oplus [-3] \oplus \bU\) \\
%  \(7\) & \(28\) & \(-12\) & \(2 [-1] \oplus [1] \oplus [-2] \oplus [-6] \oplus \bU\) \\
%  \(7\) & \(29\) & \(-12\) & \([-1] \oplus \bU \oplus [1, 1, -3, 0, 2, 1, 0, 0, 1, 2](-1)\) \\
%  \(7\) & \(30\) & \(-12\) & \([1] \oplus [-1] \oplus \bU \oplus [2, 1, 4, 0, 1, 2](-1)\) \\
%  \(7\) & \(31\) & \(-12\) & \([-1] \oplus [1] \oplus \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
%  \(7\) & \(32\) & \(-13\) & \(2 [-1] \oplus [-13] \oplus 2 \bU\) \\
%  \(7\) & \(33\) & \(-13\) & \(3 [-1] \oplus [-2, 1, 6] \oplus \bU\) \\
%  \(7\) & \(34\) & \(-14\) & \([1] \oplus [-1] \oplus [-2] \oplus [2, 1, 4](-1) \oplus \bU\) \\
%  \(7\) & \(35\) & \(-15\) & \([-3] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(7\) & \(36\) & \(-15\) & \([-1] \oplus [-3] \oplus [-5] \oplus 2 \bU\) \\
%  \(7\) & \(37\) & \(-16\) & \([-1] \oplus 2 [-2] \oplus [0, 2, 1] \oplus \bU\) \\
%  \(7\) & \(38\) & \(-16\) & \([1] \oplus [-1] \oplus [-2] \oplus [3, 1, 3](-1) \oplus \bU\) \\
%  \(7\) & \(39\) & \(-16\) & \(\bU \oplus [0, 2, -1, 0, 1, 2, 0, 1, 1, 2, 0, 0, 1, 1, 2](-1)\) \\
%  \(7\) & \(40\) & \(-16\) & \([-1] \oplus 2 [-4] \oplus 2 \bU\) \\
%  \(7\) & \(41\) & \(-16\) & \([-1] \oplus [-4] \oplus \bU \oplus [0, 2, -2, 0, 1, 1](-1)\) \\
%  \(7\) & \(42\) & \(-16\) & \(2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(7\) & \(43\) & \(-16\) & \([1] \oplus [-1] \oplus \bU \oplus [2, 1, 2, 1, 1, 6](-1)\) \\
%  \(7\) & \(44\) & \(-16\) & \(2 [-1] \oplus [-16] \oplus 2 \bU\) \\
%  \(7\) & \(45\) & \(-16\) & \([-1] \oplus 2 [-2] \oplus \bU(2) \oplus \bU\) \\
%  \(7\) & \(46\) & \(-17\) & \([-1] \oplus 2 \bU \oplus [3, 1, 6](-1)\) \\
%  \(7\) & \(47\) & \(-18\) & \([-2] \oplus \bU \oplus [0, 3, 1, 0, 1, 1, 0, 1, 0, 1](-1)\) \\
%  \(7\) & \(48\) & \(-18\) & \([-2] \oplus 2 [-3] \oplus 2 \bU\) \\
%  \(7\) & \(49\) & \(-19\) & \(2 [-1] \oplus [-19] \oplus 2 \bU\) \\
%  \(7\) & \(50\) & \(-20\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3](-2)\) \\
%  \(7\) & \(51\) & \(-20\) & \(2 \bU \oplus [3, 1, 3, 1, 1, 3](-1)\) \\
%  \(7\) & \(52\) & \(-20\) & \([2, 1, 3](-1) \oplus \bU \oplus [-2, 1, 1, 1, 0, 1](-1)\) \\
%  \(7\) & \(53\) & \(-21\) & \(2 [-1] \oplus [3] \oplus [2, 1, 4](-1) \oplus \bU\) \\
%  \(7\) & \(54\) & \(-21\) & \([-1] \oplus [1] \oplus \bU \oplus [3, 1, 3, 0, 1, 3](-1)\) \\
%  \(7\) & \(55\) & \(-22\) & \([1] \oplus [-1] \oplus \bU \oplus [2, 1, 2, 1, 0, 8](-1)\) \\
%  \(7\) & \(56\) & \(-24\) & \(2 [-1] \oplus [-6] \oplus \bU(2) \oplus \bU\) \\
%  \(7\) & \(57\) & \(-24\) & \([-1] \oplus [-2] \oplus [-12] \oplus 2 \bU\) \\
%  \(7\) & \(58\) & \(-24\) & \([1] \oplus [-1] \oplus \bU \oplus [2, 1, 4, 1, 0, 4](-1)\) \\
%  \(7\) & \(59\) & \(-24\) & \(\bU \oplus [-1, 1, 2, 1, 0, 2, 0, 1, 0, 2, 0, 0, 1, 1, 3](-1)\) \\
%  \(7\) & \(60\) & \(-24\) & \([-1] \oplus [-3] \oplus [-8] \oplus 2 \bU\) \\
%  \(7\) & \(61\) & \(-25\) & \(\bU \oplus [1, 1, -1, 0, 1, 1, 0, 1, 0, 3, 0, -1, 0, 2, 3](-1)\) \\
%  \(7\) & \(62\) & \(-27\) & \(2 [-1] \oplus [-3] \oplus [2, 1, -4] \oplus \bU\) \\
%  \(7\) & \(63\) & \(-27\) & \([-1] \oplus [1] \oplus 3 [-3] \oplus \bU\) \\
%  \(7\) & \(64\) & \(-27\) & \([-9] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(7\) & \(65\) & \(-28\) & \(2 [-1] \oplus \bU \oplus [3, 1, 3, 0, 2, -2](-1)\) \\
%  \(7\) & \(66\) & \(-28\) & \([1] \oplus [-1] \oplus [-4] \oplus [2, 1, 4](-1) \oplus \bU\) \\
%  \(7\) & \(67\) & \(-30\) & \([-2] \oplus [2, 1, -1] \oplus [2, 1, 3](-1) \oplus \bU\) \\
%  \(7\) & \(68\) & \(-32\) & \(\bU(2) \oplus \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
%  \(7\) & \(69\) & \(-32\) & \(2 [-1] \oplus [-2] \oplus \bU(4) \oplus \bU\) \\
%  \(7\) & \(70\) & \(-32\) & \([-1] \oplus \bU \oplus [0, 4, 1, 0, 1, 1, 0, 2, 0, 2](-1)\) \\
%  \(7\) & \(71\) & \(-32\) & \([-1] \oplus \bU(2) \oplus [3, 1, 3](-1) \oplus \bU\) \\
%  \(7\) & \(72\) & \(-32\) & \([-2] \oplus 2 \bU \oplus [4, 2, 5](-1)\) \\
%  \(7\) & \(73\) & \(-32\) & \([-4] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
%  \(7\) & \(74\) & \(-32\) & \([-1] \oplus [-2] \oplus [-4] \oplus \bU(2) \oplus \bU\) \\
%  \(7\) & \(75\) & \(-33\) & \([-1] \oplus [-3] \oplus [-11] \oplus 2 \bU\) \\
%  \(7\) & \(76\) & \(-36\) & \([1] \oplus \bU \oplus [2, 1, 4, 1, 0, 4, 0, -1, 1, 2](-1)\) \\
%  \(7\) & \(77\) & \(-36\) & \([1] \oplus [-1] \oplus [-12] \oplus \bA_{2} \oplus \bU\) \\
%  \(7\) & \(78\) & \(-40\) & \([-1] \oplus 2 \bU \oplus [7, 3, 7](-1)\) \\
%  \(7\) & \(79\) & \(-40\) & \([-8] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(7\) & \(80\) & \(-45\) & \([-15] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(7\) & \(81\) & \(-48\) & \([1] \oplus [-1] \oplus [-4] \oplus \bA_{2}(2) \oplus \bU\) \\
%  \(7\) & \(82\) & \(-48\) & \([-1] \oplus [1] \oplus \bU \oplus [3, 1, 3, 1, -1, 7](-1)\) \\
%  \(7\) & \(83\) & \(-48\) & \(\bU \oplus [0, 2, -1, 0, 1, 2, 0, 1, 0, 2, 0, 1, -1, 1, 4](-1)\) \\
%  \(7\) & \(84\) & \(-48\) & \([-1] \oplus [2] \oplus [-2] \oplus \bA_{2}(2) \oplus \bU\) \\
%  \(7\) & \(85\) & \(-49\) & \([-7] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
%  \(7\) & \(86\) & \(-54\) & \([-1] \oplus [-2] \oplus [9] \oplus \bA_{2} \oplus \bU\) \\
%  \(7\) & \(87\) & \(-64\) & \([0, 2, 1] \oplus \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(7\) & \(88\) & \(-64\) & \([1] \oplus \bU \oplus [3, 1, 3, 1, -1, 3, 1, 1, -1, 5](-1)\) \\
%  \(7\) & \(89\) & \(-64\) & \([1] \oplus [-1] \oplus 3 [-4] \oplus \bU\) \\
%  \(7\) & \(90\) & \(-64\) & \(\bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 3, 0, -1, 1, 3, 2](-1)\) \\
%  \(7\) & \(91\) & \(-64\) & \(2 [-1] \oplus \bU \oplus [-3, 1, 5, 1, -3, 5](-1)\) \\
%  \(7\) & \(92\) & \(-64\) & \([-1] \oplus [2] \oplus [-2] \oplus 2 [-4] \oplus \bU\) \\
%  \(7\) & \(93\) & \(-64\) & \(\bU(2) \oplus \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(7\) & \(94\) & \(-80\) & \(2 \bU \oplus [4, 2, 7, 0, 2, 4](-1)\) \\
%  \(7\) & \(95\) & \(-80\) & \(\bU(2) \oplus \bU \oplus [3, 1, 3, 1, 1, 3](-1)\) \\
%  \(7\) & \(96\) & \(-81\) & \([-3] \oplus \bU(3) \oplus \bA_{2} \oplus \bU\) \\
%  \(7\) & \(97\) & \(-96\) & \(\bU(2) \oplus \bU \oplus [2, 1, 7, 0, 1, 2](-1)\) \\
%  \(7\) & \(98\) & \(-128\) & \(\bU(4) \oplus \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
%  \(7\) & \(99\) & \(-128\) & \([-4] \oplus \bU(2) \oplus [3, 1, 3](-1) \oplus \bU\) \\
%  \(7\) & \(100\) & \(-144\) & \([1] \oplus 2 \bA_{2}(2) \oplus \bU\) \\
%  \(7\) & \(101\) & \(-162\) & \([-2] \oplus 2 [-3] \oplus \bU(3) \oplus \bU\) \\
%  \(7\) & \(102\) & \(-192\) & \([-4] \oplus [0, 2, 1] \oplus \bA_{2}(2) \oplus \bU\) \\
%  \(7\) & \(103\) & \(-243\) & \([-9] \oplus \bU \oplus [-1, 1, 2, -1, 1, 2, 1, -1, 1, 2](-1)\) \\
%  \(7\) & \(104\) & \(-256\) & \([1] \oplus [-16] \oplus \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(7\) & \(105\) & \(-256\) & \(\bU \oplus [1, 1, -1, 0, 2, 4, 0, 2, 0, 4, 0, 2, 2, 2, 6](-1)\) \\
%  \(7\) & \(106\) & \(-256\) & \([-4] \oplus \bU \oplus [3, 1, 3, -1, 1, -1, 1, -1, 1, 3](-1)\) \\
%  \(7\) & \(107\) & \(-1024\) & \(\bU \oplus [4, 2, -1, -2, 1, 7, 0, 2, 2, 4, 0, 2, 2, 0, 4](-1)\) \\
% \midrule
%  \(8\) & \(1\) & \(1\) & \(4 [-1] \oplus 2 \bU\) \\
%  \(8\) & \(2\) & \(2\) & \(3 [-1] \oplus [-2] \oplus 2 \bU\) \\
%  \(8\) & \(3\) & \(3\) & \(3 [-1] \oplus [-3] \oplus 2 \bU\) \\
%  \(8\) & \(4\) & \(3\) & \(2 [-1] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(5\) & \(4\) & \(2 [-1] \oplus 2 [-2] \oplus 2 \bU\) \\
%  \(8\) & \(6\) & \(4\) & \([-1] \oplus 2 \bU \oplus \bA_{3}\) \\
%  \(8\) & \(7\) & \(4\) & \(3 [-1] \oplus [-4] \oplus 2 \bU\) \\
%  \(8\) & \(8\) & \(5\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(8\) & \(9\) & \(5\) & \(3 [-1] \oplus [-5] \oplus 2 \bU\) \\
%  \(8\) & \(10\) & \(6\) & \(2 [-1] \oplus [-2] \oplus [-3] \oplus 2 \bU\) \\
%  \(8\) & \(11\) & \(6\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(12\) & \(7\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3](-1)\) \\
%  \(8\) & \(13\) & \(7\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
%  \(8\) & \(14\) & \(8\) & \(2 [-1] \oplus [-2] \oplus [-4] \oplus 2 \bU\) \\
%  \(8\) & \(15\) & \(8\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 3](-1)\) \\
%  \(8\) & \(16\) & \(8\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
%  \(8\) & \(17\) & \(8\) & \(2 [-1] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
%  \(8\) & \(18\) & \(8\) & \([-1] \oplus 3 [-2] \oplus 2 \bU\) \\
%  \(8\) & \(19\) & \(9\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(20\) & \(9\) & \(3 [-1] \oplus [-9] \oplus 2 \bU\) \\
%  \(8\) & \(21\) & \(9\) & \(2 [-1] \oplus 2 [-3] \oplus 2 \bU\) \\
%  \(8\) & \(22\) & \(10\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(8\) & \(23\) & \(10\) & \(2 [-1] \oplus [-2] \oplus [-5] \oplus 2 \bU\) \\
%  \(8\) & \(24\) & \(11\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 3, 0, 0, 1, 2](-1)\) \\
%  \(8\) & \(25\) & \(12\) & \(2 \bU \oplus [2, 1, 3, 1, 2, 3, 0, 1, 1, 2](-1)\) \\
%  \(8\) & \(26\) & \(12\) & \(2 [-1] \oplus [-2] \oplus [-6] \oplus 2 \bU\) \\
%  \(8\) & \(27\) & \(12\) & \([-1] \oplus 2 [-2] \oplus [-3] \oplus 2 \bU\) \\
%  \(8\) & \(28\) & \(12\) & \(2 [-1] \oplus [-3] \oplus [-4] \oplus 2 \bU\) \\
%  \(8\) & \(29\) & \(12\) & \([-3] \oplus 2 \bU \oplus \bA_{3}\) \\
%  \(8\) & \(30\) & \(12\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
%  \(8\) & \(31\) & \(13\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 7](-1)\) \\
%  \(8\) & \(32\) & \(13\) & \(3 [-1] \oplus [-13] \oplus 2 \bU\) \\
%  \(8\) & \(33\) & \(14\) & \([-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 1, 3](-1)\) \\
%  \(8\) & \(34\) & \(15\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 3, 1, 0, 0, 3](-1)\) \\
%  \(8\) & \(35\) & \(15\) & \(2 [-1] \oplus 2 \bU \oplus [4, 1, 4](-1)\) \\
%  \(8\) & \(36\) & \(16\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 3, 0, 1, 1, 2](-1)\) \\
%  \(8\) & \(37\) & \(16\) & \(2 [-1] \oplus [-2] \oplus [-8] \oplus 2 \bU\) \\
%  \(8\) & \(38\) & \(16\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 3](-1)\) \\
%  \(8\) & \(39\) & \(16\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 3, 1, 1, 1, 3](-1)\) \\
%  \(8\) & \(40\) & \(16\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 1, 1, 5](-1)\) \\
%  \(8\) & \(41\) & \(16\) & \([-1] \oplus 2 [-2] \oplus [-4] \oplus 2 \bU\) \\
%  \(8\) & \(42\) & \(17\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 0, 4](-1)\) \\
%  \(8\) & \(43\) & \(18\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus [2, 1, 5](-1)\) \\
%  \(8\) & \(44\) & \(18\) & \([-1] \oplus [-6] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(45\) & \(19\) & \(2 \bU \oplus [2, 1, 3, 1, 0, 3, 0, 1, 0, 2](-1)\) \\
%  \(8\) & \(46\) & \(20\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3, 1, 1, 3](-1)\) \\
%  \(8\) & \(47\) & \(20\) & \([-1] \oplus 2 [-2] \oplus [-5] \oplus 2 \bU\) \\
%  \(8\) & \(48\) & \(20\) & \([-1] \oplus 2 \bU \oplus [2, 1, 6, 0, 1, 2](-1)\) \\
%  \(8\) & \(49\) & \(20\) & \([-1] \oplus [-4] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(8\) & \(50\) & \(21\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
%  \(8\) & \(51\) & \(21\) & \(3 [-1] \oplus [-21] \oplus 2 \bU\) \\
%  \(8\) & \(52\) & \(22\) & \(2 [-1] \oplus [-2] \oplus [-11] \oplus 2 \bU\) \\
%  \(8\) & \(53\) & \(24\) & \([-2] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
%  \(8\) & \(54\) & \(24\) & \(2 \bU \oplus [2, 1, 3, 1, 0, 3, 0, 1, 1, 3](-1)\) \\
%  \(8\) & \(55\) & \(24\) & \([-1] \oplus [-8] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(56\) & \(24\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
%  \(8\) & \(57\) & \(24\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus \bA_{2}(2)\) \\
%  \(8\) & \(58\) & \(25\) & \([-1] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(8\) & \(59\) & \(27\) & \(2 [-3] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(60\) & \(27\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 3, 1, 0, 1, 3](-1)\) \\
%  \(8\) & \(61\) & \(27\) & \(2 \bU \oplus [2, 1, 5](-1) \oplus \bA_{2}\) \\
%  \(8\) & \(62\) & \(28\) & \([-1] \oplus 2 [-2] \oplus [-7] \oplus 2 \bU\) \\
%  \(8\) & \(63\) & \(28\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 6](-1)\) \\
%  \(8\) & \(64\) & \(30\) & \(2 [-1] \oplus [-3] \oplus [-10] \oplus 2 \bU\) \\
%  \(8\) & \(65\) & \(32\) & \([-4] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
%  \(8\) & \(66\) & \(32\) & \([-1] \oplus [-4] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
%  \(8\) & \(67\) & \(32\) & \(2 [-1] \oplus 2 \bU \oplus [3, 1, 3](-2)\) \\
%  \(8\) & \(68\) & \(32\) & \(2 [-1] \oplus [-2] \oplus [-16] \oplus 2 \bU\) \\
%  \(8\) & \(69\) & \(32\) & \([-1] \oplus [-2] \oplus 2 [-4] \oplus 2 \bU\) \\
%  \(8\) & \(70\) & \(32\) & \(2 [-2] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
%  \(8\) & \(71\) & \(32\) & \(2 \bU \oplus [3, 1, 3, -1, 1, 3, -1, 1, 1, 3](-1)\) \\
%  \(8\) & \(72\) & \(33\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 1, 9](-1)\) \\
%  \(8\) & \(73\) & \(33\) & \([-1] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 5](-1)\) \\
%  \(8\) & \(74\) & \(35\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 7, 0, 0, 1, 2](-1)\) \\
%  \(8\) & \(75\) & \(36\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus \bA_{2}(2)\) \\
%  \(8\) & \(76\) & \(36\) & \([-1] \oplus 2 \bU \oplus [2, 1, 10, 0, 1, 2](-1)\) \\
%  \(8\) & \(77\) & \(36\) & \([-3] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 2](-1)\) \\
%  \(8\) & \(78\) & \(40\) & \(2 \bU \oplus [2, 1, 3](-1) \oplus [3, 1, 3](-1)\) \\
%  \(8\) & \(79\) & \(40\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 6](-1)\) \\
%  \(8\) & \(80\) & \(42\) & \([-2] \oplus [-7] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(81\) & \(44\) & \(2 \bU \oplus [2, 1, 3, 0, 1, 2, 0, 1, 0, 6](-1)\) \\
%  \(8\) & \(82\) & \(45\) & \([-1] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 5](-1)\) \\
%  \(8\) & \(83\) & \(48\) & \([-3] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 3](-1)\) \\
%  \(8\) & \(84\) & \(48\) & \(2 \bU \oplus [3, 1, 3, 1, -1, 3, 1, 1, -1, 4](-1)\) \\
%  \(8\) & \(85\) & \(48\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 7, 0, 1, 1, 2](-1)\) \\
%  \(8\) & \(86\) & \(48\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 5, 1, 1, -1, 5](-1)\) \\
%  \(8\) & \(87\) & \(48\) & \([-1] \oplus 2 [-2] \oplus [-12] \oplus 2 \bU\) \\
%  \(8\) & \(88\) & \(48\) & \(2 \bU \oplus [3, 1, 3, 1, 1, 3, 1, 1, 1, 3](-1)\) \\
%  \(8\) & \(89\) & \(51\) & \(2 \bU \oplus [2, 1, 3, 0, 1, 6, 0, 0, 1, 2](-1)\) \\
%  \(8\) & \(90\) & \(54\) & \([-2] \oplus 3 [-3] \oplus 2 \bU\) \\
%  \(8\) & \(91\) & \(56\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 4, 1, 0, 1, 4](-1)\) \\
%  \(8\) & \(92\) & \(60\) & \([-1] \oplus 2 [-2] \oplus [-15] \oplus 2 \bU\) \\
%  \(8\) & \(93\) & \(64\) & \([-8] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
%  \(8\) & \(94\) & \(64\) & \(2 [-2] \oplus 2 \bU \oplus [4, 2, 5](-1)\) \\
%  \(8\) & \(95\) & \(64\) & \([-4] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 3](-1)\) \\
%  \(8\) & \(96\) & \(72\) & \(2 \bU \oplus [2, 1, 6, 0, 1, 3, 0, 1, -1, 3](-1)\) \\
%  \(8\) & \(97\) & \(80\) & \(2 \bU \oplus [2, 1, 7, 0, 1, 2, 0, 2, 0, 4](-1)\) \\
%  \(8\) & \(98\) & \(80\) & \([-4] \oplus 2 \bU \oplus [3, 1, 3, 1, 1, 3](-1)\) \\
%  \(8\) & \(99\) & \(81\) & \([-3] \oplus [-9] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(100\) & \(81\) & \(2 [-3] \oplus 2 \bU \oplus [2, 1, 5](-1)\) \\
%  \(8\) & \(101\) & \(96\) & \([-4] \oplus 2 \bU \oplus [2, 1, 7, 0, 1, 2](-1)\) \\
%  \(8\) & \(102\) & \(96\) & \(2 \bU \oplus [3, 1, 3](-1) \oplus \bA_{2}(2)\) \\
%  \(8\) & \(103\) & \(108\) & \(2 \bU \oplus [2, 1, 7, 0, 1, 2, 0, 3, 0, 6](-1)\) \\
%  \(8\) & \(104\) & \(108\) & \([-2] \oplus 2 [-3] \oplus [-6] \oplus 2 \bU\) \\
%  \(8\) & \(105\) & \(112\) & \([-7] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(8\) & \(106\) & \(125\) & \([-1] \oplus 3 [-5] \oplus 2 \bU\) \\
%  \(8\) & \(107\) & \(128\) & \(2 \bU \oplus [2, 1, 7, -1, 2, 7, 0, 1, 1, 2](-1)\) \\
%  \(8\) & \(108\) & \(128\) & \([-2] \oplus 2 \bU \oplus [4, 2, 5, 2, 1, 5](-1)\) \\
%  \(8\) & \(109\) & \(128\) & \([-1] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 3](-2)\) \\
%  \(8\) & \(110\) & \(128\) & \(2 [-4] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
%  \(8\) & \(111\) & \(135\) & \(2 \bU \oplus \bA_{2} \oplus [2, 1, 3](-3)\) \\
%  \(8\) & \(112\) & \(144\) & \([-3] \oplus [-4] \oplus 2 \bU \oplus \bA_{2}(2)\) \\
%  \(8\) & \(113\) & \(162\) & \([-6] \oplus [-9] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(8\) & \(114\) & \(192\) & \([-1] \oplus 2 \bU \oplus [2, 1, 7, 0, 1, 2](-2)\) \\
%  \(8\) & \(115\) & \(192\) & \([-3] \oplus 3 [-4] \oplus 2 \bU\) \\
%  \(8\) & \(116\) & \(216\) & \(2 \bU \oplus \bA_{2} \oplus [3, 1, 3](-3)\) \\
%  \(8\) & \(117\) & \(240\) & \([-15] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(8\) & \(118\) & \(243\) & \(2 \bU \oplus [2, 1, 5](-1) \oplus \bA_{2}(-3)\) \\
%  \(8\) & \(119\) & \(256\) & \(2 \bU \oplus [4, 2, 7, 0, 2, 4, 0, 2, 0, 4](-1)\) \\
%  \(8\) & \(120\) & \(432\) & \(2 [-3] \oplus 2 \bU \oplus \bA_{2}(-4)\) \\
%  \(8\) & \(121\) & \(512\) & \(2 \bU \oplus [4, 2, 7, 2, 3, 7, 2, 3, -1, 7](-1)\) \\
%  \(8\) & \(122\) & \(768\) & \(2 \bU \oplus [4, 2, 15, 0, 2, 4, 0, 2, 0, 4](-1)\) \\
% \midrule
%  \(9\) & \(1\) & \(-1\) & \(5 [-1] \oplus 2 \bU\) \\
%  \(9\) & \(2\) & \(-2\) & \(4 [-1] \oplus [-2] \oplus 2 \bU\) \\
%  \(9\) & \(3\) & \(-3\) & \(4 [-1] \oplus [-3] \oplus 2 \bU\) \\
%  \(9\) & \(4\) & \(-3\) & \(3 [-1] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(9\) & \(5\) & \(-4\) & \(2 [-1] \oplus 2 \bU \oplus \bA_{3}\) \\
%  \(9\) & \(6\) & \(-4\) & \(3 [-1] \oplus 2 [-2] \oplus 2 \bU\) \\
%  \(9\) & \(7\) & \(-5\) & \(3 [-1] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(9\) & \(8\) & \(-5\) & \(4 [-1] \oplus [-5] \oplus 2 \bU\) \\
%  \(9\) & \(9\) & \(-6\) & \(3 [-1] \oplus [-2] \oplus [-3] \oplus 2 \bU\) \\
%  \(9\) & \(10\) & \(-6\) & \(4 [-1] \oplus [-6] \oplus 2 \bU\) \\
%  \(9\) & \(11\) & \(-7\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3](-1)\) \\
%  \(9\) & \(12\) & \(-8\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 0, 0, 3](-1)\) \\
%  \(9\) & \(13\) & \(-8\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
%  \(9\) & \(14\) & \(-8\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus \bA_{3}\) \\
%  \(9\) & \(15\) & \(-9\) & \(4 [-1] \oplus [-9] \oplus 2 \bU\) \\
%  \(9\) & \(16\) & \(-9\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 1, 2, 1, 1, 0, 0, 3](-1)\) \\
%  \(9\) & \(17\) & \(-9\) & \([-1] \oplus 2 \bU \oplus 2 \bA_{2}\) \\
%  \(9\) & \(18\) & \(-10\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 4](-1)\) \\
%  \(9\) & \(19\) & \(-11\) & \(4 [-1] \oplus [-11] \oplus 2 \bU\) \\
%  \(9\) & \(20\) & \(-11\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3, 0, 0, 1, 2](-1)\) \\
%  \(9\) & \(21\) & \(-12\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 3, 0, 0, 0, 1, 2](-1)\) \\
%  \(9\) & \(22\) & \(-12\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
%  \(9\) & \(23\) & \(-12\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3, 0, 1, -1, 2](-1)\) \\
%  \(9\) & \(24\) & \(-12\) & \(2 [-1] \oplus 2 [-2] \oplus [-3] \oplus 2 \bU\) \\
%  \(9\) & \(25\) & \(-14\) & \(2 [-1] \oplus [-2] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
%  \(9\) & \(26\) & \(-14\) & \([-1] \oplus [-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3](-1)\) \\
%  \(9\) & \(27\) & \(-15\) & \(2 [-1] \oplus [-5] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(9\) & \(28\) & \(-15\) & \(2 [-1] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(9\) & \(29\) & \(-16\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 3, 1, 1, 1, 3, 0, 0, 1, -1, 2](-1)\) \\
%  \(9\) & \(30\) & \(-16\) & \([-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 1, 1, 3](-1)\) \\
%  \(9\) & \(31\) & \(-16\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3, 0, 1, 1, 2](-1)\) \\
%  \(9\) & \(32\) & \(-17\) & \(4 [-1] \oplus [-17] \oplus 2 \bU\) \\
%  \(9\) & \(33\) & \(-18\) & \(3 [-1] \oplus [-3] \oplus [-6] \oplus 2 \bU\) \\
%  \(9\) & \(34\) & \(-20\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 6, 0, 1, 2](-1)\) \\
%  \(9\) & \(35\) & \(-20\) & \(2 [-1] \oplus [-4] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(9\) & \(36\) & \(-20\) & \([-1] \oplus 2 [-2] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(9\) & \(37\) & \(-21\) & \(2 [-1] \oplus [-7] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(9\) & \(38\) & \(-23\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 3, 0, 1, 5](-1)\) \\
%  \(9\) & \(39\) & \(-24\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 3, 1, 0, 1, 0, 4](-1)\) \\
%  \(9\) & \(40\) & \(-24\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 0, 0, 7](-1)\) \\
%  \(9\) & \(41\) & \(-24\) & \(2 [-1] \oplus [-3] \oplus 2 \bU \oplus [3, 1, 3](-1)\) \\
%  \(9\) & \(42\) & \(-24\) & \(2 [-1] \oplus [-2] \oplus [-3] \oplus [-4] \oplus 2 \bU\) \\
%  \(9\) & \(43\) & \(-25\) & \(3 [-1] \oplus 2 [-5] \oplus 2 \bU\) \\
%  \(9\) & \(44\) & \(-26\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 4](-1)\) \\
%  \(9\) & \(45\) & \(-27\) & \(3 [-1] \oplus [-3] \oplus [-9] \oplus 2 \bU\) \\
%  \(9\) & \(46\) & \(-27\) & \([-1] \oplus 2 \bU \oplus \bA_{2} \oplus [2, 1, 5](-1)\) \\
%  \(9\) & \(47\) & \(-28\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3, 1, 0, 0, 3](-1)\) \\
%  \(9\) & \(48\) & \(-29\) & \(4 [-1] \oplus [-29] \oplus 2 \bU\) \\
%  \(9\) & \(49\) & \(-30\) & \(2 [-1] \oplus [-6] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(9\) & \(50\) & \(-32\) & \([-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 3, 1, 0, 1, 3](-1)\) \\
%  \(9\) & \(51\) & \(-32\) & \([-2] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 2, 1, 1, 1, 5](-1)\) \\
%  \(9\) & \(52\) & \(-32\) & \(2 \bU \oplus [2, 1, 3, 1, 0, 3, 1, 2, 1, 4, 0, 1, -1, 1, 2](-1)\) \\
%  \(9\) & \(53\) & \(-35\) & \(2 [-1] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
%  \(9\) & \(54\) & \(-36\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 3, 1, 0, 1, 4, 0, 0, 1, 0, 2](-1)\) \\
%  \(9\) & \(55\) & \(-36\) & \(2 [-1] \oplus 2 [-3] \oplus [-4] \oplus 2 \bU\) \\
%  \(9\) & \(56\) & \(-36\) & \([-1] \oplus 2 [-2] \oplus 2 [-3] \oplus 2 \bU\) \\
%  \(9\) & \(57\) & \(-39\) & \(2 [-1] \oplus [-13] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(9\) & \(58\) & \(-40\) & \(2 [-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 0, 14](-1)\) \\
%  \(9\) & \(59\) & \(-41\) & \(4 [-1] \oplus [-41] \oplus 2 \bU\) \\
%  \(9\) & \(60\) & \(-44\) & \([-1] \oplus 2 \bU \oplus [2, 1, 2, 1, 1, 3, 1, 0, 0, 7](-1)\) \\
%  \(9\) & \(61\) & \(-44\) & \(2 [-1] \oplus 2 [-2] \oplus [-11] \oplus 2 \bU\) \\
%  \(9\) & \(62\) & \(-45\) & \(3 [-1] \oplus 2 \bU \oplus [2, 1, 3](-3)\) \\
%  \(9\) & \(63\) & \(-48\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 3, 0, 0, 1, 2, 0, 0, 0, 1, 5](-1)\) \\
%  \(9\) & \(64\) & \(-48\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(9\) & \(65\) & \(-48\) & \([-1] \oplus [-4] \oplus 2 \bU \oplus [2, 1, 3, 1, 1, 3](-1)\) \\
%  \(9\) & \(66\) & \(-50\) & \(2 \bU \oplus [2, 1, 3](-1) \oplus [2, 1, 2, 1, 0, 4](-1)\) \\
%  \(9\) & \(67\) & \(-54\) & \([-1] \oplus [-2] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 5](-1)\) \\
%  \(9\) & \(68\) & \(-54\) & \(3 [-1] \oplus [-6] \oplus [-9] \oplus 2 \bU\) \\
%  \(9\) & \(69\) & \(-56\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 3, 1, 0, 0, 3, 0, -1, 1, 0, 3](-1)\) \\
%  \(9\) & \(70\) & \(-56\) & \(2 \bU \oplus [2, 1, 4](-1) \oplus [2, 1, 3, 0, 1, 2](-1)\) \\
%  \(9\) & \(71\) & \(-60\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3](-1) \oplus \bA_{2}(2)\) \\
%  \(9\) & \(72\) & \(-63\) & \([-7] \oplus 2 \bU \oplus 2 \bA_{2}\) \\
%  \(9\) & \(73\) & \(-64\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 4, 1, 1, 2, 4, 0, 1, 1, 1, 2](-1)\) \\
%  \(9\) & \(74\) & \(-65\) & \(3 [-1] \oplus 2 \bU \oplus [2, 1, 33](-1)\) \\
%  \(9\) & \(75\) & \(-72\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 3, 1, 0, 1, 3, 1, 1, 0, 1, 6](-1)\) \\
%  \(9\) & \(76\) & \(-75\) & \([-5] \oplus 2 \bU \oplus [2, 1, 3](-1) \oplus \bA_{2}\) \\
%  \(9\) & \(77\) & \(-80\) & \([-2] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 3, 0, -1, 1, 3](-1)\) \\
%  \(9\) & \(78\) & \(-80\) & \([-1] \oplus 2 [-4] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(9\) & \(79\) & \(-81\) & \([-9] \oplus 2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 1, 3](-1)\) \\
%  \(9\) & \(80\) & \(-84\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 8, 0, 1, 0, 2, 0, 1, 1, 0, 2](-1)\) \\
%  \(9\) & \(81\) & \(-90\) & \([-1] \oplus [-2] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 8](-1)\) \\
%  \(9\) & \(82\) & \(-96\) & \([-1] \oplus [-3] \oplus 2 \bU \oplus [3, 1, 3, 1, -1, 5](-1)\) \\
%  \(9\) & \(83\) & \(-96\) & \([-2] \oplus 2 \bU \oplus [2, 1, 4, 0, 1, 3, 0, 1, 1, 3](-1)\) \\
%  \(9\) & \(84\) & \(-96\) & \(2 \bU \oplus [3, 1, 3](-1) \oplus [2, 1, 4, 0, 1, 2](-1)\) \\
%  \(9\) & \(85\) & \(-104\) & \(2 \bU \oplus [2, 1, 4, 0, 1, 5, 0, 0, 1, 2, 0, 0, 1, 0, 2](-1)\) \\
%  \(9\) & \(86\) & \(-108\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 1, 0, 7, 1, 1, 0, -2, 7](-1)\) \\
%  \(9\) & \(87\) & \(-108\) & \(2 [-1] \oplus [-3] \oplus 2 \bU \oplus [2, 1, 5](-2)\) \\
%  \(9\) & \(88\) & \(-117\) & \([-1] \oplus 2 \bU \oplus [2, 1, 20](-1) \oplus \bA_{2}\) \\
%  \(9\) & \(89\) & \(-120\) & \([-1] \oplus 2 \bU \oplus [2, 1, 3](-1) \oplus [4, 2, 7](-1)\) \\
%  \(9\) & \(90\) & \(-125\) & \([-1] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 5, 0, 1, 3](-1)\) \\
%  \(9\) & \(91\) & \(-128\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 3, 1, 1, 1, 4, 1, 0, 0, 1, 4](-1)\) \\
%  \(9\) & \(92\) & \(-135\) & \(2 \bU \oplus \bA_{2} \oplus [2, 1, 5, 1, 2, 6](-1)\) \\
%  \(9\) & \(93\) & \(-140\) & \(2 [-2] \oplus [-5] \oplus 2 \bU \oplus [2, 1, 4](-1)\) \\
%  \(9\) & \(94\) & \(-144\) & \([-1] \oplus [-6] \oplus [-8] \oplus 2 \bU \oplus \bA_{2}\) \\
%  \(9\) & \(95\) & \(-144\) & \([-1] \oplus 2 [-3] \oplus 2 [-4] \oplus 2 \bU\) \\
%  \(9\) & \(96\) & \(-176\) & \([-1] \oplus [-11] \oplus 2 \bU \oplus [3, 1, 3, -1, 1, 3](-1)\) \\
%  \(9\) & \(97\) & \(-189\) & \([-7] \oplus 2 \bU \oplus [2, 1, 5](-1) \oplus \bA_{2}\) \\
%  \(9\) & \(98\) & \(-192\) & \(2 \bU \oplus [2, 1, 3, 1, 1, 4, -1, 0, 1, 4, 0, 0, 1, -1, 5](-1)\) \\
%  \(9\) & \(99\) & \(-200\) & \(2 \bU \oplus [2, 1, 2, 1, 1, 7, 1, 1, 2, 7, 0, 0, 1, 1, 2](-1)\) \\
%  \(9\) & \(100\) & \(-216\) & \(2 \bU \oplus [2, 1, 6, 0, 1, 3, 0, 1, -1, 3, 0, 1, 1, 1, 4](-1)\) \\
%  \(9\) & \(101\) & \(-216\) & \(2 \bU \oplus [2, 1, 2, 1, 0, 3, 1, 0, 0, 6, 1, 0, 1, -2, 8](-1)\) \\
%  \(9\) & \(102\) & \(-300\) & \([-2] \oplus [-5] \oplus [-6] \oplus 2 \bU \oplus [2, 1, 3](-1)\) \\
%  \(9\) & \(103\) & \(-320\) & \(2 \bU \oplus [2, 1, 4, 1, 2, 4, 0, -1, 1, 5, 0, -1, 1, 1, 5](-1)\) \\
%  \(9\) & \(104\) & \(-360\) & \([-3] \oplus 2 \bU \oplus [2, 1, 8](-1) \oplus [3, 1, 3](-1)\) \\
%  \(9\) & \(105\) & \(-384\) & \(2 \bU \oplus [3, 1, 3, -1, 1, 6, 0, 0, 1, 4, 0, 0, 2, 2, 4](-1)\) \\
%  \(9\) & \(106\) & \(-432\) & \([-3] \oplus 2 \bU \oplus [3, 1, 4, 1, 0, 4, 1, 0, 0, 4](-1)\) \\
%  \(9\) & \(107\) & \(-441\) & \([-21] \oplus 2 \bU \oplus [2, 1, 2, 1, 1, 2, 1, 0, 0, 6](-1)\) \\
%  \(9\) & \(108\) & \(-560\) & \(2 \bU \oplus [2, 1, 4](-1) \oplus [4, 2, 7, 0, 2, 4](-1)\) \\
%  \(9\) & \(109\) & \(-576\) & \([-1] \oplus 2 \bU \oplus [6, 3, 7, -3, 1, 7, 3, 0, 0, 7](-1)\) \\
%  \(9\) & \(110\) & \(-1200\) & \(2 \bU \oplus [3, 1, 4, 1, 0, 4, 1, 2, 2, 7, 1, 2, 2, 2, 8](-1)\) \\
% \midrule
%  \(10\) & \(1\) & \(1\) & \(2 [1] \oplus \bE_{8}\) \\
%  \(10\) & \(2\) & \(2\) & \([1] \oplus [2] \oplus \bE_{8}\) \\
%  \(10\) & \(3\) & \(3\) & \([1] \oplus [3] \oplus \bE_{8}\) \\
%  \(10\) & \(4\) & \(4\) & \([1] \oplus [4] \oplus \bE_{8}\) \\
%  \(10\) & \(5\) & \(5\) & \([1] \oplus [5] \oplus \bE_{8}\) \\
%  \(10\) & \(6\) & \(6\) & \([1] \oplus [6] \oplus \bE_{8}\) \\
%  \(10\) & \(7\) & \(7\) & \([1] \oplus [7] \oplus \bE_{8}\) \\
%  \(10\) & \(8\) & \(8\) & \([1] \oplus [8] \oplus \bE_{8}\) \\
%  \(10\) & \(9\) & \(9\) & \([1] \oplus [9] \oplus \bE_{8}\) \\
%  \(10\) & \(10\) & \(10\) & \([1] \oplus [10] \oplus \bE_{8}\) \\
%  \(10\) & \(11\) & \(12\) & \([1] \oplus [12] \oplus \bE_{8}\) \\
%  \(10\) & \(12\) & \(13\) & \([1] \oplus [13] \oplus \bE_{8}\) \\
%  \(10\) & \(13\) & \(15\) & \([1] \oplus [15] \oplus \bE_{8}\) \\
%  \(10\) & \(14\) & \(16\) & \([1] \oplus [16] \oplus \bE_{8}\) \\
%  \(10\) & \(15\) & \(18\) & \([1] \oplus [18] \oplus \bE_{8}\) \\
%  \(10\) & \(16\) & \(21\) & \([1] \oplus [21] \oplus \bE_{8}\) \\
%  \(10\) & \(17\) & \(22\) & \([1] \oplus [22] \oplus \bE_{8}\) \\
%  \(10\) & \(18\) & \(24\) & \([1] \oplus [24] \oplus \bE_{8}\) \\
%  \(10\) & \(19\) & \(25\) & \([1] \oplus [25] \oplus \bE_{8}\) \\
%  \(10\) & \(20\) & \(28\) & \([1] \oplus [28] \oplus \bE_{8}\) \\
%  \(10\) & \(21\) & \(30\) & \([1] \oplus [30] \oplus \bE_{8}\) \\
%  \(10\) & \(22\) & \(33\) & \([1] \oplus [33] \oplus \bE_{8}\) \\
%  \(10\) & \(23\) & \(37\) & \([1] \oplus [37] \oplus \bE_{8}\) \\
%  \(10\) & \(24\) & \(40\) & \([1] \oplus [40] \oplus \bE_{8}\) \\
%  \(10\) & \(25\) & \(42\) & \([1] \oplus [42] \oplus \bE_{8}\) \\
%  \(10\) & \(26\) & \(45\) & \([1] \oplus [45] \oplus \bE_{8}\) \\
%  \(10\) & \(27\) & \(48\) & \([1] \oplus [48] \oplus \bE_{8}\) \\
%  \(10\) & \(28\) & \(57\) & \([1] \oplus [57] \oplus \bE_{8}\) \\
%  \(10\) & \(29\) & \(58\) & \([1] \oplus [58] \oplus \bE_{8}\) \\
%  \(10\) & \(30\) & \(60\) & \([1] \oplus [60] \oplus \bE_{8}\) \\
%  \(10\) & \(31\) & \(70\) & \([1] \oplus [70] \oplus \bE_{8}\) \\
%  \(10\) & \(32\) & \(72\) & \([1] \oplus [72] \oplus \bE_{8}\) \\
%  \(10\) & \(33\) & \(78\) & \([1] \oplus [78] \oplus \bE_{8}\) \\
%  \(10\) & \(34\) & \(85\) & \([1] \oplus [85] \oplus \bE_{8}\) \\
%  \(10\) & \(35\) & \(88\) & \([1] \oplus [88] \oplus \bE_{8}\) \\
%  \(10\) & \(36\) & \(93\) & \([1] \oplus [93] \oplus \bE_{8}\) \\
%  \(10\) & \(37\) & \(102\) & \([1] \oplus [102] \oplus \bE_{8}\) \\
%  \(10\) & \(38\) & \(105\) & \([1] \oplus [105] \oplus \bE_{8}\) \\
%  \(10\) & \(39\) & \(112\) & \([1] \oplus [112] \oplus \bE_{8}\) \\
%  \(10\) & \(40\) & \(120\) & \([1] \oplus [120] \oplus \bE_{8}\) \\
%  \(10\) & \(41\) & \(130\) & \([1] \oplus [130] \oplus \bE_{8}\) \\
%  \(10\) & \(42\) & \(133\) & \([1] \oplus [133] \oplus \bE_{8}\) \\
%  \(10\) & \(43\) & \(165\) & \([1] \oplus [165] \oplus \bE_{8}\) \\
%  \(10\) & \(44\) & \(168\) & \([1] \oplus [168] \oplus \bE_{8}\) \\
%  \(10\) & \(45\) & \(177\) & \([1] \oplus [177] \oplus \bE_{8}\) \\
%  \(10\) & \(46\) & \(190\) & \([1] \oplus [190] \oplus \bE_{8}\) \\
%  \(10\) & \(47\) & \(210\) & \([1] \oplus [210] \oplus \bE_{8}\) \\
%  \(10\) & \(48\) & \(232\) & \([1] \oplus [232] \oplus \bE_{8}\) \\
%  \(10\) & \(49\) & \(240\) & \([1] \oplus [240] \oplus \bE_{8}\) \\
%  \(10\) & \(50\) & \(253\) & \([1] \oplus [253] \oplus \bE_{8}\) \\
%  \(10\) & \(51\) & \(273\) & \([1] \oplus [273] \oplus \bE_{8}\) \\
%  \(10\) & \(52\) & \(280\) & \([1] \oplus [280] \oplus \bE_{8}\) \\
%  \(10\) & \(53\) & \(312\) & \([1] \oplus [312] \oplus \bE_{8}\) \\
%  \(10\) & \(54\) & \(330\) & \([1] \oplus [330] \oplus \bE_{8}\) \\
%  \(10\) & \(55\) & \(345\) & \([1] \oplus [345] \oplus \bE_{8}\) \\
%  \(10\) & \(56\) & \(357\) & \([1] \oplus [357] \oplus \bE_{8}\) \\
%  \(10\) & \(57\) & \(385\) & \([1] \oplus [385] \oplus \bE_{8}\) \\
%  \(10\) & \(58\) & \(408\) & \([1] \oplus [408] \oplus \bE_{8}\) \\
%  \(10\) & \(59\) & \(462\) & \([1] \oplus [462] \oplus \bE_{8}\) \\
%  \(10\) & \(60\) & \(520\) & \([1] \oplus [520] \oplus \bE_{8}\) \\
%  \(10\) & \(61\) & \(760\) & \([1] \oplus [760] \oplus \bE_{8}\) \\
%  \(10\) & \(62\) & \(840\) & \([1] \oplus [840] \oplus \bE_{8}\) \\
%  \(10\) & \(63\) & \(1320\) & \([1] \oplus [1320] \oplus \bE_{8}\) \\
%  \(10\) & \(64\) & \(1365\) & \([1] \oplus [1365] \oplus \bE_{8}\) \\
%  \(10\) & \(65\) & \(1848\) & \([1] \oplus [1848] \oplus \bE_{8}\) \\
% \midrule
%  \(11\) & \(1\) & \(-1\) & \([1] \oplus \bU \oplus \bE_{8}\) \\


\end{longtable}

\end{center}

